Towards Effectively Leveraging Execution Traces for Program Repair with Code LLMs

Large Language Models (LLMs) show promising performance on various programming tasks, including Automatic Program Repair (APR). However, most approaches to LLM-based APR are limited to the static analysis of the programs, while disregarding their runtime behavior. Inspired by knowledge-augmented NLP, in this work, we aim to remedy this potential blind spot by augmenting standard APR prompts with program execution traces. We evaluate our approach using the GPT family of models on three popular APR datasets. Our findings suggest that simply incorporating execution traces into the prompt provides a limited performance improvement over trace-free baselines, in only 2 out of 6 tested dataset / model configurations. We further find that the effectiveness of execution traces for APR diminishes as their complexity increases. We explore several strategies for leveraging traces in prompts and demonstrate that LLM-optimized prompts help outperform trace-free prompts more consistently. Additionally, we show trace-based prompting to be superior to finetuning a smaller LLM on a small-scale dataset; and conduct probing studies reinforcing the notion that execution traces can complement the reasoning abilities of the LLMs.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> sections/discussion.tex <==
\section{Discussion: Is fine-tuning a better option than Prompting?}

==> sections/error_analysis.tex <==
\begin{table*}[t]
  \centering
  \caption{\textbf{Error Analysis for Trace-based and Error-based Prompts. AA = Assignment Addition, CMP=Comparison, AEM=Assignment Expression Modification, BCM= Branch Condition Modification, CBA=Condition Branch Addition, CBD=Condition Branch Deletion, CEE= Condition Expression Expansion, CEM=Condition Expression Modification, IM=Initialization Modification, LCM=Loop Condition Modification, MOM=Math Operator Modification ,MCA=Method Call Addition, MCM=Method Call Modification, MCPM=Method Call Parameter Modification, REM= Return Expression Modification , TM= Type Modification, VM=Variable Modification, CBM=Condition Branch Modification, DSA=Declaration Statement Addition, MCPA=Method Call Parameter Addition, MCPD= Method Call Parameter Deletion}}
%\label{tab:Per_c10_2}
  \resizebox{0.98\textwidth}{!}{
    \begin{tabular}{c|cl|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|}
    \toprule
    Model & Dataset & CMP& AA & AEM & BCM&   CBA &  CBD &  CEE &  CEM &  IM&  LCM & MOM & MCA & MCM& MCPM &REM&TM &VM& CBM&DSA&MCPA&MCPD\\
    \midrule
    \multirow{8}[1]{*}{GPT-3.5} & \multirow{4}[1]{*}{Refactory} & EP>TP &   \ApplyColorIfNeeded{0}  &   \ApplyColorIfNeeded{0}   &   \ApplyColorIfNeeded{0}    &  \ApplyColorIfNeeded{0}   &   \ApplyColorIfNeeded{0}    &   \ApplyColorIfNeeded{0}   &  \ApplyColorIfNeeded{0}     & \ApplyColorIfNeeded{0}      &  \ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{0} &\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}\\
    &  & TP>EP &        \ApplyColorIfNeeded{0}  &   \ApplyColorIfNeeded{0}   &   \ApplyColorIfNeeded{0}    &  \ApplyColorIfNeeded{0}   &   \ApplyColorIfNeeded{0}    &   \ApplyColorIfNeeded{0}   &  \ApplyColorIfNeeded{0}     & \ApplyColorIfNeeded{0}      &  \ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{0} &\ApplyColorIfNeeded{2}& \ApplyColorIfNeeded{2}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}   &\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}\\ 
    
    &  & FSE>FST & \ApplyColorIfNeeded{0}  &   \ApplyColorIfNeeded{0}   &   \ApplyColorIfNeeded{1}    &  \ApplyColorIfNeeded{0}   &   \ApplyColorIfNeeded{0}    &   \ApplyColorIfNeeded{0}   &  \ApplyColorIfNeeded{0}     & \ApplyColorIfNeeded{1}      &  \ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{1} &\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{2}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}\\
     &  & FST>FSE &       \ApplyColorIfNeeded{0}  &   \ApplyColorIfNeeded{0}   &   \ApplyColorIfNeeded{0}    &  \ApplyColorIfNeeded{0}   &   \ApplyColorIfNeeded{0}    &   \ApplyColorIfNeeded{0}   &  \ApplyColorIfNeeded{0}     & \ApplyColorIfNeeded{0}      &  \ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{0} &\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}\\
\cline{2-23}

    
     & \multirow{4}[1]{*}{HumanEvalJ} &  EP>TP &   \ApplyColorIfNeeded{0}  &   \ApplyColorIfNeeded{1}   &   \ApplyColorIfNeeded{0}    &  \ApplyColorIfNeeded{1}   &   \ApplyColorIfNeeded{0}    &   \ApplyColorIfNeeded{0}   &  \ApplyColorIfNeeded{3}     & \ApplyColorIfNeeded{0}      &  \ApplyColorIfNeeded{2}&\ApplyColorIfNeeded{1}& \ApplyColorIfNeeded{3} &\ApplyColorIfNeeded{1}& \ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{0}\\
    &  & TP>EP &        \ApplyColorIfNeeded{0}  &   \ApplyColorIfNeeded{0}   &   \ApplyColorIfNeeded{0}    &  \ApplyColorIfNeeded{1}   &   \ApplyColorIfNeeded{1}    &   \ApplyColorIfNeeded{1}   &  \ApplyColorIfNeeded{1}     & \ApplyColorIfNeeded{0}      &  \ApplyColorIfNeeded{2}&\ApplyColorIfNeeded{2}& \ApplyColorIfNeeded{2} &\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{3}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{3}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{1}\\ 
    
    &  & FSE>FST & \ApplyColorIfNeeded{0}  &   \ApplyColorIfNeeded{2}   &   \ApplyColorIfNeeded{0}    &  \ApplyColorIfNeeded{2}   &   \ApplyColorIfNeeded{0}    &   \ApplyColorIfNeeded{2}   &  \ApplyColorIfNeeded{3}     & \ApplyColorIfNeeded{0}      &  \ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{1}& \ApplyColorIfNeeded{2} &\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{4}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{2}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{0}\\
     &  & FST>FSE &       \ApplyColorIfNeeded{0}  &   \ApplyColorIfNeeded{1}   &   \ApplyColorIfNeeded{0}    &  \ApplyColorIfNeeded{1}   &   \ApplyColorIfNeeded{0}    &   \ApplyColorIfNeeded{0}   &  \ApplyColorIfNeeded{2}     & \ApplyColorIfNeeded{3}      &  \ApplyColorIfNeeded{2}&\ApplyColorIfNeeded{3}& \ApplyColorIfNeeded{2} &\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{2}&\ApplyColorIfNeeded{3}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}\\
     \midrule
     \multirow{8}[1]{*}{GPT-4} & \multirow{4}[1]{*}{Refactory} & EP>TP &   \ApplyColorIfNeeded{0}  &   \ApplyColorIfNeeded{0}   &   \ApplyColorIfNeeded{0}    &  \ApplyColorIfNeeded{0}   &   \ApplyColorIfNeeded{0}    &   \ApplyColorIfNeeded{0}   &  \ApplyColorIfNeeded{0}     & \ApplyColorIfNeeded{0}      &  \ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{0} &\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}\\
    &  & TP>EP &        \ApplyColorIfNeeded{0}  &   \ApplyColorIfNeeded{0}   &   \ApplyColorIfNeeded{0}    &  \ApplyColorIfNeeded{0}   &   \ApplyColorIfNeeded{0}    &   \ApplyColorIfNeeded{0}   &  \ApplyColorIfNeeded{0}     & \ApplyColorIfNeeded{0}      &  \ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{0} &\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}   &\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}\\ 
    
    &  & FSE>FST & \ApplyColorIfNeeded{0}  &   \ApplyColorIfNeeded{0}   &   \ApplyColorIfNeeded{1}    &  \ApplyColorIfNeeded{0}   &   \ApplyColorIfNeeded{0}    &   \ApplyColorIfNeeded{0}   &  \ApplyColorIfNeeded{0}     & \ApplyColorIfNeeded{1}      &  \ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{2} &\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}\\
     &  & FST>FSE &       \ApplyColorIfNeeded{0}  &   \ApplyColorIfNeeded{0}   &   \ApplyColorIfNeeded{0}    &  \ApplyColorIfNeeded{0}   &   \ApplyColorIfNeeded{0}    &   \ApplyColorIfNeeded{0}   &  \ApplyColorIfNeeded{0}     & \ApplyColorIfNeeded{0}      &  \ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{0} &\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}\\
\cline{2-23}

    
     & \multirow{4}[1]{*}{HumanEvalJ} & EP>TP &   \ApplyColorIfNeeded{1}  &   \ApplyColorIfNeeded{1}   &   \ApplyColorIfNeeded{0}    &  \ApplyColorIfNeeded{3}   &   \ApplyColorIfNeeded{1}    &   \ApplyColorIfNeeded{1}   &  \ApplyColorIfNeeded{1}     & \ApplyColorIfNeeded{2}      &  \ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{2} &\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}\\
    &  & TP>EP &     \ApplyColorIfNeeded{0}  &  \ApplyColorIfNeeded{1}  &   \ApplyColorIfNeeded{1}    &  \textcolor{white}{\ApplyColorIfNeeded{6}}   &  \ApplyColorIfNeeded{1}  &    \ApplyColorIfNeeded{0}   &  \ApplyColorIfNeeded{2}    & \ApplyColorIfNeeded{2}      &  \ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{1} &\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{3}&\ApplyColorIfNeeded{2}&\ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}\\
    &  & FSE>FST &     \ApplyColorIfNeeded{1}  &   \ApplyColorIfNeeded{2}    &   \ApplyColorIfNeeded{1}    &  \ApplyColorIfNeeded{1}     &   \ApplyColorIfNeeded{0}    &    \ApplyColorIfNeeded{1}   &  \ApplyColorIfNeeded{2}     & \ApplyColorIfNeeded{4}      &  \ApplyColorIfNeeded{4}&\ApplyColorIfNeeded{2}& \ApplyColorIfNeeded{0} &\ApplyColorIfNeeded{1}& \ApplyColorIfNeeded{2}&\ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{3}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}\\
     &  & FST>FSE &     \ApplyColorIfNeeded{1}  &   \ApplyColorIfNeeded{0}    &   \ApplyColorIfNeeded{0}    &  \ApplyColorIfNeeded{2}     &   \ApplyColorIfNeeded{1}    &    \ApplyColorIfNeeded{0}   &  \ApplyColorIfNeeded{1}     & \ApplyColorIfNeeded{2}      &  \ApplyColorIfNeeded{2}&\ApplyColorIfNeeded{1}& \ApplyColorIfNeeded{2} &\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}\\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:RQ3}%
\end{table*}%

==> sections/evaluation.tex <==
\label{sec:eval}
We aim to answer four research question with our evaluation.

\noindent\textbf{RQ1.} Are prompts with deterministic traces more effective at solving bugs than prompts without execution traces?

\noindent\textbf{RQ2.} How trace complexity affects the effectiveness of trace-based prompts?

\noindent\textbf{RQ3.} Can the format of traces be optimized to guarantee gains for APR?

\noindent\textbf{RQ4.} Is fine-tuning a better option than prompting for program repair?
\subsection{Set Up}
\noindent\textbf{Datasets.} 
In our search for evaluation datasets, we performed an extensive survey covering 15 popular datasets for Python, Java, C++ and other major languages. The main differentiators were dataset size and program diversity, availability of unit tests, and the origin of the dataset i.e. either self-contained algorithmic problems (e.g., CodeNet \cite{}) or complete open source projects (e.g., PyTraceBugs \cite{}). While using the most realistic datasets would be ideal, being able to execute them in order to evaluate a bug presents a considerable challenge and even setting up the dependencies requires substantial manual effort on a project by project basis.
On the other hand, algorithmic datasets offer important practical advantages such as manageable length, easily testable self-contained functions, which is especially relevant for being able to generate traces via execution. 

We chose the following three APR datasets: Refactory~\cite{hu2019re}, RunBugRun~\cite{prenner2023runbugrun}, and Humaneval-Java~\cite{jiang2023impact}. 
Refactory consists of nearly 2000 faulty Python programs submitted by students, across 5 distinct algorithmic problems.
Given the high ratio in the number of buggy solutions for any given problem, by evaluating on this dataset we hope to account for the full range of possible mistakes in each algorithm.
RunBugRun is a APR oriented derivative of the expansive CodeNet code competitions dataset, comprising nearly a quarter of million submissions encompassing 4000 distinct problems. 
To keep the number of evaluated programs manageable we uniformly sampled 1000 bugs from the Python validation split.
HumanEval is a well-known dataset of around 160 hand-written programs purpose built for evaluating program generation, originally in Python but later ported to other popular languages \cite{chen2021evaluating}. 
For the purpose of testing APR performance we use a variant derived from it called HumanEval-Java \cite{jiang2023impact}, in which diverse bugs are synthetically injected into the programs. 

Each problem in all of the datasets came with at least 5 test cases.
For RunBugRun, given that inputs are fed via standard input and output via print statement, we implemented a wrapper that pipes input to the script and then captures standard output into a variable to be compared with the ground truth value.

\noindent\textbf{Models.} With the landscape of state-of-the-art code LLMs rapidly changing, we chose use two most widely studied commercial models from OpenAI for ease of comparison with other work: GPT-3.5 Turbo ~\cite{ouyang2022training} and GPT-4~\cite{OpenAI2023GPT4TR}. 
These two models represent two different performance tiers both in terms of the number of parameters and different release timelines, hence, studying these models could shine the light on the LLMs' evolving ability to reason about program execution across product generations. While there is undoubtedly scope for including more proprietary as well as open source models, given our narrow focus on traces, we leave this to be explored in future work.

%\noindent\textbf{Prompt Types.} To understand the effectiveness of execution traces in the GPT model for APR, we feed various prompts (including and excluding execution traces) to GPT models. First type of prompts are called \textit{\textbf{Program Prompts (PP)}}, in which the faulty program is fed to the GPT models without any additional details. in the second type of prompts, we include test case assertion errors in the prompt together with the faulty program (\textbf{PP+Error} ). These prompts are called \textit{\textbf{Error Prompts (EP)}}. Third type of prompts are called \textit{\textbf{Trace Prompts (TP)}}, where we include execution trace along with faulty program and assertion error in the prompt (\textbf{PP+Error+Trace}). 

%To improve the prompt effectiveness, we use few-shot (FS) prompts with both errors and traces. These prompts are called few-shot error (FSE) prompts and few-shot trace (FST) prompts. In these prompts, we first randomly select five examples from the dataset and randomly use three of the examples in the prompt. For FSE, the examples include faulty program, assertion error and correct program. While for FST, the examples also include execution traces (\textbf{FSE+Trace}). 

%Each of the prompts only includes a single program with a single test case. Although we understand that having multiple test-cases in a single program can have a better possibility in repairing a program, our objective in the work is to find the effect of adding execution traces to the prompt. Hence, we only create prompts where we can show the evaluation with both including and excluding traces. If we were to use multiple test cases in a prompt, that might lead to having multiple execution traces in the prompt, which can lead to prompts exceeding maximum context length.  

%Additionally, we use enriched prompts like chain-of-thought prompting  with traces (COTT) and extended few shot prompts with traces (FST-Ext) to measure if enriched prompts can improve the program repairing capability of trace prompts or not. For COTT, we modify the instruction in the FST prompts to first find the location of the bug rather than provide a fix in one shot. The response to that prompt is then chained with the instruction to provide a fix based on the bug location predicted at the previous step. For FST-Ext, we extend the few-shot examples to include the trace of the correct program execution in addition to the failing one.


%For chain-of-thought prompting (COTT), we modify the instruction in the FST prompts to first find the location of the bug rather than provide a fix on one shot. The response to that prompt is then chained with the instruction to provide a fix based on the bug location predicted at the previous step.

%Additionally, we use extended few shot prompts with traces (FST-Ext), which extends the few-shot examples to include the trace of the correct program execution in addition to the failing one. The intuition behind using the correct trace is that GPT model might be able to understand the failing execution traces better if both correct and wrong traces are provided in the example. 
\noindent\textbf{Prompt Types.} We consider all the prompt types discussed in Section \ref{sec:method} , including error-based prompts. The prompts are referred to by using the following terms: Deterministic Trace Prompts (DTP), Error Prompts (EP), Collated Trace Prompts (CTP), LLM-summarized Trace Prompts (STP), and Conditional Selection of Traces (CST).



\noindent\textbf{Baselines.} %We consider all the prompt types discussed in Section \ref{sec:method}, including error prompts (EP).
% We follow prompt format from Xia et al. (~\citeyear{ICSE10172803}).
% To ensure the prompt and response fit within the GPT model context-size, we truncate the content of the prompt if the number of lines exceeds 200.
%  All the used prompts can be found at: https://anonymous.4open.science/r/CodePlanGPT-DBF3/. Additionally, we have added an example of all the prompts in Section \ref{sec:prompt} in the Appendix.
We consider the following baselines:

\noindent\textit{Prompt-based baseline}: with this baseline, we explore prompting LLMs using execution traces generated by them (instead of actual program execution traces). This is inspired by Self-Debugging~\cite{chen2023teaching} where LLMs are prompted to debug their own generated code. In particular, we draw inspirations from the \textit{Explanation} step of this work where the model is asked to generate execution traces for a predicted code. In our prompts, we provide LLMs with a program and a test case feedback, and ask them to first, trace through the execution of the program and determine the needed fix, and then correct the function accordingly. We perform these experiments with both GPT3.5 and GPT4.0.

\noindent\textit{Training-based baseline}: here, we explore how finetuning a model using execution traces performs in fixing the errors. This approach is inspired by TraceFixer~\cite{bouzenia2023tracefixer} which finetunes a CodeT5 model using the buggy program's code, its execution trace and the desired state of program.
% and SelfAPR~\cite{ye2022selfapr} (which trains a neural model using execution traces)
We use the prompts that include execution traces to finetune deepseek-coder-1.3b-instruct~\footnote{https://github.com/deepseek-ai/DeepSeek-Coder}. We use the training setting and parameters suggested by the model developers to finetune this model, and the input to the model consist of buggy programs, failing test case results and execution traces. For each dataset, 80\% of the problems are used for training and the rest are reserved for testing.

Refactory finetuning: trained on Qs 3, 4,5, and tested on Qs 1 and 2. 
Used "Refactored correct code" for the correct version, in total, in 172 cases this column was null so we skipped those cases. 
in the end: 291 training examples, and 116 testing examples.
% \end{enumerate}






%that have faulty program, assertion errors, and execution traces in the prompt. We name these prompts as \textit{\textbf{Trace Prompts (TP)}}. Additionally, we use two different types of prompts as baselines to compare prompts with execution traces.  For the first baseline, we include test case assertion errors in the prompt together with the faulty program but not the execution trace. These prompts are referred to as \textit{\textbf{Error Prompts (EP)}}. For both EP and TP, we create multiple combinations between unique faulty programs from the dataset and corresponding unit test cases.In the second baseline, we do not provide any additional information other than the faulty program in the prompt. We refer these kind of prompts as \textit{\textbf{Program Prompts (PP)}}. 

\noindent\textbf{Metrics.} 
In previous work on APR, models are evaluated either at the granularity of distinct bugs solved cf. -- \cite{ICSE10172803}, \cite{jiang2023impact} or individual test cases passed \cite{tian2023chatgpt}.
In both cases, the model is prompted once with each buggy program, and results are aggregated from multiple output samples from the APR model.
In our case, we obtain multiple prompts for a given program -- each one specific to a particular failing test case and the corresponding execution trace.
Rather than aggregating from multiple sampled predictions, we obtain a single prediction for each test case-specific prompt and aggregate them across prompts when computing the metrics. %, while setting the GPT model's temperature parameter to 0. 
For this setup the most meaningful metrics are 
% To make our results comparable to previous work, we report accuracy at the level of individual test cases, generated fixes, and finally unique buggy programs.
% We use three metrics to explore the GPT model's capability to reason about execution traces. 
%\textit{\textbf{Correct Test Accuracy (CTA)}} evaluates the percentage of unit test cases that are correct using at least one of the GPT-generated fixes.
%We report accuracy of the LLM using two metrics. 
\textit{\textbf{Correct Fix Accuracy (CFA)}}, which is the percentage generated fixes that successfully pass all test cases; and \textit{\textbf{Correct Program Accuracy (CPA)}}, which groups multiple fixes generated for a given program and measures the percentage of programs that have at least one correct fix. We do not separately report testcase-level accuracy as that is too lenient with respect to partially working fixes and does not take into account the disparity in the number of test cases for each program.

% To illustrate, let's assume the dataset has 10 faulty programs, each with 5 unit test cases (50 unique test cases). For Error Prompts (EP) and Trace Prompts (TP), 50 different prompts are created, which are fed to a GPT model. GPT model would generate 50 corresponding program fixes. Those 50 program fixes are evaluated on 5 unit test cases. 
% %If 25 of the 50 unique test cases are passed by at least one fix, then CTA would be (25/50)*100=50\%. 
% If out of 50 program fixes, 10 programs pass all 5 test cases, the CFA would be (10/50)*100=25\%. Also, if there are five programs out of 10 faulty programs for which at least one program is generated that passes all unit test cases, then CPA would be (5/10)*100=50\%.

% \begin{comment}
% \begin{figure*}[!t]
%     \centering
% \begin{subfigure}[b]{0.45\textwidth}
%         \includegraphics[width=\textwidth]{figures/GPT35_HEJ.pdf}
%         \caption{HumanEval-Java Dataset with GPT-3.5 }
%          \label{fig:HEJ_GPT35}
%     \end{subfigure}
%     % \begin{subfigure}[b]{0.355\textwidth}
%     %     \includegraphics[width=\textwidth]{figures/corruption_skipnet.pdf}
%     %     \caption{Effect of corruption on SkipNet}
%     % \end{subfigure}
%     \begin{subfigure}[b]{0.45\textwidth}
%         \includegraphics[width=\textwidth]{figures/GPT4_HEJ.pdf}
%         \caption{HumanEval-Java Dataset with GPT-4}
%         \label{fig:HEJ_GPT4}
%     \end{subfigure}

%     \begin{subfigure}[b]{0.45\textwidth}
%         \includegraphics[width=\textwidth]{figures/GPT35_REF.pdf}
%         \caption{Refactory Dataset with GPT-3.5 }
%          \label{fig:REF_GPT35}
%     \end{subfigure}
%     % \begin{subfigure}[b]{0.355\textwidth}
%     %     \includegraphics[width=\textwidth]{figures/corruption_skipnet.pdf}
%     %     \caption{Effect of corruption on SkipNet}
%     % \end{subfigure}
%     \begin{subfigure}[b]{0.45\textwidth}
%         \includegraphics[width=\textwidth]{figures/GPT4_REF.pdf}
%         \caption{Refactory Dataset with GPT-4}
%         \label{fig:REF_GPT4}
%     \end{subfigure}
%      \caption{CPA, CFA, and CTA values for different prompts. 'CPA', 'CFA', and  'CTA' are represented by  'skyblue',  'lightgreen',  'salmon' color bars respectively.}
%     \label{fig:acc}
% \end{figure*}




% \end{comment}
% \begin{table*}[t]
%   \centering
%   \caption{\textbf{Quantitative Results for Using Different Prompts. FP = Faulty Programs,  CF = Correct Fixes, CP = Correct Programs, CFA = Correct Fix Accuracy and CPA = Correct Program Accuracy. }}
% \label{tab:Per_c10_2_2}
%   \resizebox{0.8\textwidth}{!}{
%     \begin{tabular}{c|cl|r|r|r|r|r|r}
%     \toprule
%     Model & Dataset & Method & $\#$ FPs &  $\#$ Fixes &   $\#$ CF &  $\#$ CP  &  CFA & CPA\\
%     \midrule
%         \multirow{12}[1]{*}{GPT-3.5} & \multirow{6}[1]{*}{Refactory} & Self-Debug &     \multirow{6}[1]{*}{138}  &   \multirow{6}[1]{*}{579}    &   244    &  73     &  0.421     &    0.529   \\
%           &       & EP &        &       &    304  &   91    &  0.525    &    0.659    \\
%           &       & DTP &        &       &  295   &  87     &   0.509    &    0.630      \\
%           &       & CTP &       &       &    262  &  81     &   0.452    &   0.587    \\
%           &       & STP &        &       &   291   &  83     & 0.502     &  0.601     \\
%           &       & CST &        &       &    213  &  53     &  0.368     &  0.384      \\
%           \cline{2-9}
%           &\multirow{6}[1]{*}{HumanEval-Java}  & Self-Debug &     \multirow{6}[1]{*}{157}  &   \multirow{6}[1]{*}{634}    &   210    &  75     &   0.331    &   0.477    \\
%           &       & EP &        &       &  241    &   85    & 0.380     &   0.541     \\
%           &       & DTP &        &       &   212  &  86     &  0.334     &   0.547       \\
%           &       & CTP &       &       &   248   &  78     &  0.391     &   0.497    \\
%           &       & STP &        &       &  273    &  84     & 0.430     &   0.535    \\
%           &       & CST &        &       &   241   &  82     & 0.380      &  0.522      \\
%           \cline{2-9}
%           &\multirow{6}[1]{*}{RunBugRun}& Self-Debug &     \multirow{6}[1]{*}{456}  &   \multirow{6}[1]{*}{559}    &   151    &  132     &  0.270     &    0.289   \\
%           &       & EP &        &       &  260    &   221    & 0.465     &    0.484    \\
%           &       & DTP &        &       &  249   &  216     &  0.445     &     0.473     \\
%           &       & CTP &       &       &   213   &  186     &   0.381    &    0.407   \\
%           &       & STP &        &       &  264    &  227     &  0.472    &   0.497    \\
%           &       & CST &        &       &  240    &  207     &   0.429    &   0.453     \\
%           \midrule

%     \multirow{12}[1]{*}{GPT-4} & \multirow{6}[1]{*}{Refactory}   & Self-Debug&  \multirow{6}[1]{*}{138}    &   \multirow{6}[1]{*}{579}    &  414     &  117     &  0.715  & 0.847  \\
%           &       & EP &        &       &   458   &   122    &  0.791    &    0.884    \\
%           &       & DTP &        &       &  427   &  113     &  0.737     &       0.818   \\
%           &       & CTP &       &       &   380   &  113     &  0.656     &    0.818    \\
%           &       & STP &        &       &  436    &  119     & 0.753   &     0.862   \\
%           &       & CST &        &       &   426   &  117     & 0.735      &   0.847      \\
%           \cline{2-9}
%           &\multirow{6}[1]{*}{HumanEval-Java} & Self-Debug&   \multirow{6}[1]{*}{157}    &   \multirow{6}[1]{*}{634}    &  312     &   105    & 0.492   &0.668   \\
%           &       & EP &        &       &   313   &   104    & 0.493     &    0.662    \\
%           &       & DTP &        &       &  324   &  112     &   0.511    &    0.713      \\
%           &       & CTP &       &       &    337  &    107   &   0.531    &    0.681   \\
%           &       & STP &        &       &  363    &  112     &  0.572    &   0.713    \\
%           &       & CST &        &       &   348   &  115     &  0.549     &      0.732  \\
%           \cline{2-9}
%           &\multirow{6}[1]{*}{RunBugRun} & Self-Debug   &   \multirow{6}[1]{*}{456}  &   \multirow{6}[1]{*}{559}&  337     &   287    & 0.602   & 0.629   \\
%           &       & EP &        &       & 296     &   264    &  0.529    &   0.578     \\
%           &       & DTP &        &       &   312  &  266     &    0.558   &   0.583       \\
%           &       & CTP &       &       &   270   &  232     &   0.483    &  0.508     \\
%           &       & STP &        &       & 319     &  269     & 0.570     &    0.589   \\
%           &       & CST &        &       &  295    &  251     &  0.527     &   0.550     \\
%     \bottomrule
%     \end{tabular}%
%     }
%   \label{tab:addlabel_2}%
% \end{table*}%






% Both metrics have significance in quantifying GPT model's capability for program repair. CFA is important to find out the percentage of correct programs generated by GPT models. But, it is possible that GPT model is generating multiple correct fixes for one faulty program, while for other faulty programs, none of the generated fixes are correct. Hence, CPA measurement also becomes important.

\begin{comment}
\begin{figure*}
  \begin{center}
    \includegraphics[width=0.8\textwidth]{figures/Findings-GPT3.5.drawio-2.pdf}
  \end{center}
  \caption{Venn diagrams showing fixed programs which are solved only using different error-based and trace-based prompts (For GPT-3.5 model and HumanEval-Java dataset.)}
  \label{fig:rq3_java_gpt3.5}
\end{figure*}
\end{comment}
\subsection{RQ1. Are prompts with deterministic traces more effective at solving bugs than prompts without execution traces?}
 \begin{comment}
     \multirow{1}[2]{*}{Model} & \multirow{1}[2]{*}{Dataset} & \multicolumn{1}{c|}{\multirow{1}[2]{*}{Prompt Type}} & \multicolumn{1}{c|}{# of Faulty Programs} & \multicolumn{1}{c|}{# of Prompts} & \multicolumn{1}{c|}{# of Test Cases} & \multicolumn{1}{c|}{# of Correct Programs} & \multicolumn{1}{c|}{# of Correct Unique Programs} & \multicolumn{1}{c}{# of Correct Test Cases} &  \multicolumn{1}{c}{CTA}&  \multicolumn{1}{c}{CPA} & \multicolumn{1}{c}{CUPA}\\
 \end{comment}
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[h!]
\centering
\caption{Quantitative Results for RQ1. Bold indicates a winning configuration for a given model and dataset. Italic indicates a runner up configuration.}
\begin{tabular}{lllrrrr}
Dataset   Name                   & Prompt Type                            & Model                         & \textbf{\#FP}           & \textbf{\#Fixes}        & \textbf{CFA}                 & \textbf{CPA}                 \\ \hline
\multirow{6}[1]{*}{Refactory}                        & Baseline                               & \multirow{3}[1]{*}{GPT3.5}                        & 137                     & 573                     & 0.425829                     & 0.532847                     \\
                        & Error Prompt                           &                         & 138                     & 577                     & \textbf{0.526863  }                   & \textbf{0.65942}                      \\
                        & Trace Prompt                           &                         & 138                     & 579                     & 0.509499                     & 0.630435                     \\ 
                        \cline{2-7}
                        & Baseline                               & \multirow{3}[1]{*}{GPT4}                          & 137                     & 573                     & 0.722513                     & 0.854015                     \\
                        & Error Prompt                           &                           & 137                     & 573                     & \textbf{0.799302}                     & \textbf{0.890511}                     \\
                        & Trace Prompt                           &                           & 136                     & 561                     & 0.761141                     & 0.830882                     \\ \hline
\multirow{6}[1]{*}{HEJ}                              & Baseline                               & \multirow{3}[1]{*}{GPT3.5}                        & 157                     & 634                     & 0.33123                      & 0.477707                     \\
                              & Error Prompt                           &                        & 157                     & 634                     & \textbf{0.380126}                     & 0.541401                     \\
                              & Trace Prompt                           &                        & 157                     & 634                     & 0.334385                     & \textbf{0.547771}                     \\ \cline{2-7}
                              & Baseline                               & \multirow{3}[1]{*}{GPT4}                          & 157                     & 634                     & 0.492114                     & 0.66879                      \\
                              & Error Prompt                           &                           & 157                     & 634                     & 0.493691                     & 0.66242                      \\
                              & Trace Prompt                           &                           & 157                     & 634                     & \textbf{0.511041}                     & \textbf{0.713376}                     \\ \hline
\multirow{6}[1]{*}{rbugr}                          & Baseline                               & \multirow{3}[1]{*}{GPT3.5}                        & 456                     & 558                     & 0.270609                     & 0.289474                     \\
                            & Error Prompt                           &                        & 456                     & 559                     & \textbf{0.465116}                     & \textbf{0.484649}                     \\
                            & Trace Prompt                           &                      & 453                     & 555                     & \textit{0.448649}                     & \textit{0.476821}                     \\ \cline{2-7}
                            & Baseline                               & \multirow{3}[1]{*}{GPT4}                        & 456                     & 559                     & \textbf{0.602862}                     & \textbf{0.629386}                     \\
                            & Error Prompt                           &                           & 456                     & 559                     & 0.529517                     & 0.578947                     \\
                            & Trace Prompt                           &                           & 453                     & 554                     & \textit{0.563177}                     & \textit{0.587196}                     \\ \hline             
\end{tabular}
\end{table*}
In this research question, our objective is to evaluate the effectiveness of including deterministic program execution traces into LLM prompts, for solving APR tasks. Our two points of comparison are the prompt augmented with just the failing test case, and the prompt containing an instruction to generate program's execution trace before providing a fix, in the style of the Self-Debug work.
The effectiveness is measured through reporting CPA and CFA. 

%with and without execution traces in the prompt. To evaluate the effectiveness, we use three metrics (CPA, CFA, and CTA) on the responses generated by aforementioned prompts. The objective is to determine the effectiveness of added traces in the prompts. Hence, we mainly compare PP-EP-TP and FSE-FST results. 

%We first discuss about different used prompt-types and then discuss the evaluation results.


%We have used multiple types of prompts for TP and EP, which are discussed in details during exploring the RQs.

The evaluation results can be found in Table \ref{tab:addlabel_2}). The number of faulty programs, number of fixes and total test cases is the same for all types of prompts per each dataset.  

Across the board, the Self-Debug baseline performs the worst except in one configuration using GPT-4 on the run\_bug\_run dataset. This outcome is unsurprising as having the LLM generate an execution trace could be introducing hallucination and thus undermining the resulting fixes.
For both GPT 3.5 and 4 on the Refactory dataset, prompts including just a failing test case decisively outperform ones with execution traces by multiple percentage points on both fix accuracy and program accuracy. 
On the HumanEval-Java dataset with GPT 3.5 error-only prompts are only ahead in terms of fix accuracy but slightly behind in program accuracy. Whereas with GPT 4, trace-based prompts consistently outperform error-only prompts on both metrics. 
Results on run\_bug\_run paint a similar picture, where GPT 3.5 doesn't seem to benefit from including traces, while GPT 4 gets a tangible lift over the error-only prompts. 
Overall, on two out of three datasets, trace-based prompts significantly improve the ability of GPT-4 to generate working bug fixes. 
While GPT 3.5 lagging behind terms of absolute scores irrespective or prompt type is expected,  more broadly its inability to benefit from execution traces (even degraded performance) could highlight a qualitative generational gap, when it comes to emergent abilities of LLMs. 
Notwithstanding, there still remain a few unexplained results for example, the lack of performance gain from using traces on the Refactory dataset and the unusually strong performance of the Self-Debug baseline in one particular configuration. To gain a fine grained understanding, in the next research question, we focus on studying the varying complexity of execution traces and how it affects downstream APR performance.




% For HumanEval-Java dataset, for both GPT-3.5 and GPT-4, DTP-generated responses have higher CPA than self-apr and EP generated responses; showing that more unique programs can be fixed if traces are added. However for GPT-3.5, CFA is lower for TP with comparison to EP. Self-apr performs worst w.r.t both CPA and CFA.

% For Refactory dataset, the EP-generated responses performs best with both CPA and CFA. Self-apr mostly performs worst among the three techniques, however, for GPT-4 model, it can be found that CPA of DTP-generated responses is lower than self-apr. 

% Additionally for RunBugRun dataset, selfapr-generated responses show best CPA and CFA for GPT-3.5 model, whereas for GPT-4 model they perform worst. The performance of EP-generated response and DTP-generated responses is similar considering both metrics.
% Hence, it can be said that both trace-based prompting techniques (DTP and self-apr) do not perform consistently across datasets and across metrics. Specifically, self-apr performs workst among three techniques suggesting that GPT generated execution traces might not be reliable. Also, inconsistent performance of DTP calls for additional investigation regarding the techniques performance.


%However, in comparison between FSE and FST generated responses, we could find that adding few-shot examples can improve the error-based prompts significantly. However, adding few-shot examples to trace-based prompts could create large prompts, which can lead to a generation of more unusable responses (dropping the CPA). Also, using COTT and FST-Ext does not help trace-based prompts significantly, as this leads to larger prompts and more unusable responses.

%One interesting observation is that having a higher CFA does not always lead to a higher CPA. These results indicate that a type of prompt could generate multiple correct fixes for one faulty program, showing higher CFA but lower CPA.

%For the Refractory dataset, for the GPT-3.5 model, TP-generated responses repair a higher number of faulty programs than EP-generated responses; however, for GPT-4, the numbers remain the same. Similar to the findings for the HumanEval-Java dataset, for Refractory also, FST prompts fail to improve CPA more than FSE prompts.

%The first notable observation is that the number of faulty programs is not the same for all types of prompts. This is because of some of the responses generated by GPT model did not contain a valid fix and were thus discarded as unusable.

%For GPT-3.5 model and Refactory dataset, program prompt (PP) can generate 40 correct fixes that repair 40 programs. However, using error prompt (EP) or trace prompt (TP) improves the program repairing capability of GPT-3.5 significantly --- with more than double the CFA and CPA rates. With respect to CFA, EP performs approximately 3\% better than TP. However, w.r.t CPA, TP can generate more correct programs than PP and EP. The results indicate that EP could generate multiple correct fixes for one faulty program, but EP and TP's capability to generate fixes for different faulty programs is similar.




%For GPT-3.5 model and HumanEval-Java dataset, program prompt (PP) can not generate any correct fixes, surprisingly. However, using EP and TP significantly improves the capability of the GPT model. While CTA for TP is higher than EP, the CFA for EP is higher than TP. However, having a better percentage of correct fixes does not lead to having a better percentage of correct programs (CPA). TP helps to fix one program more than EP, given same number of faulty programs. Based on the results of both datasets, it is evident that execution traces do not help to improve GPT-3.5 in repairing programs. 



%For GPT-4 model, we could find different trends in our findings. For Refactory dataset, TP has lower effectiveness than EP w.r.t CTA and CPA. However, for HumanEval-Java dataset, TP performs extensively well by improving program repairing capability in GPT-4. TP could repair 112 programs (8 higher than EP generated correct programs) with a CPA of 72.2\%. These results suggest that for HumanEval-Java dataset, GPT-4 potentially relied on program execution traces to repair programs. One reason behind these contrastive results might be because of the formation of both datasets. Refactory is collected based on wrong programming assignment answers where the bug in the program might not be understood correctly with execution traces (\textit{e.g.,} missing return statement). While, the HumanEval-Java dataset is created by modifying existing lines of a correct program, where execution traces can provide a better idea of the bug.
\begin{center}
\begin{tcolorbox}[colback=gray!10,%gray background
                  colframe=black,% black frame colour
                  width=7.5cm,% Use 8cm total width,
                  arc=1mm, auto outer arc,
                  boxrule=0.9pt,
                 ]
 \textbf{RQ1 Summary.} Deterministic Trace-based Prompts do not consistently perform better than error prompts for repairing programs. 
\end{tcolorbox}
\end{center}


%\subsubsection{Set Up}


%\noindent\textbf{Evaluation Results.} The evaluation results can be found in Table \ref{tab:addlabel}. For Refactory dataset, few-shot examples do not improve the performance of GPT model for neither GPT-3.5 nor GPT-4 models (For both EP and TP). However FSE and FST prompts do not decrease the GPT model's program repairing capability either. By contrast, for the HumanEval-Java dataset, for both EP and TP, the program repair capability of GPT models increases significantly. 

%On the other hand, using chain-of-thought (COTT) and extended traces (FST-Ext) do not improve the program repairing capability of GPT model's on any datasets. For GPT-3.5 model, we could find significant drop in CPA by using COTT and FST-Ext prompts. For FST-Ext prompts, one of the reasons behind these results is because of longer few-shot prompt examples. Because of longer few-shot prompt examples, fewer examples could be added to the prompt, decreasing the few-shot capability.

\begin{comment}
\begin{center}
\begin{tcolorbox}[colback=gray!10,%gray background
                  colframe=black,% black frame colour
                  width=7.5cm,% Use 8cm total width,
                  arc=1mm, auto outer arc,
                  boxrule=0.9pt,
                 ]
 \textbf{RQ2 Summary.} Adding Few-shot examples do not improve the model's capability to repair programs always. Also, chain-of-thought prompting does not help in improving model capability.
\end{tcolorbox}
\end{center}
\end{comment}
\subsection{RQ2. How are trace complexity and LLM performance related?}
\todo[author=Miraz]{Add the modified RQ2 here.}

\begin{figure}[!t]
    \centering
% \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=0.45\textwidth]{figures/hej_gpt4_trceanly.pdf}
        \caption{HumanEval-Java Dataset with GPT-4 }
         \label{fig:HEJ_GPT4}
    % \end{subfigure}
    % \begin{subfigure}[b]{0.355\textwidth}
    %     \includegraphics[width=\textwidth]{figures/corruption_skipnet.pdf}
    %     \caption{Effect of corruption on SkipNet}
    % \end{subfigure}
    % \begin{subfigure}[b]{0.45\textwidth}
    %     \includegraphics[width=\textwidth]{figures/hej_gpt35_trceanly.pdf}
    %     \caption{HumanEval-Java Dataset with GPT-3.5}
    %     \label{fig:HEJ_GPT35}
    % \end{subfigure}

    % \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=0.45\textwidth]{figures/rbr_gpt4_trceanly.pdf}
        \caption{RunBugRun Dataset with GPT-4 }
         \label{fig:RBR_GPT4}
    % \end{subfigure}
    % \begin{subfigure}[b]{0.355\textwidth}
    %     \includegraphics[width=\textwidth]{figures/corruption_skipnet.pdf}
    %     \caption{Effect of corruption on SkipNet}
    % \end{subfigure}
    % \begin{subfigure}[b]{0.45\textwidth}
    %     \includegraphics[width=\textwidth]{figures/rbr_gpt35_trceanly.pdf}
    %     \caption{Refactory Dataset with GPT-3.5}
    %     \label{fig:RBR_GPT35}
    % \end{subfigure}

    % \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=0.45\textwidth]{figures/ref_gpt4_trceanly.pdf}
        \caption{Refactory Dataset with GPT-4 }
         \label{fig:REF_GPT4}
    % \end{subfigure}
    % \begin{subfigure}[b]{0.355\textwidth}
    %     \includegraphics[width=\textwidth]{figures/corruption_skipnet.pdf}
    %     \caption{Effect of corruption on SkipNet}
    % \end{subfigure}
    % \begin{subfigure}[b]{0.45\textwidth}
    %     \includegraphics[width=\textwidth]{figures/ref_gpt35_trceanly.pdf}
    %     \caption{Refactory Dataset with GPT-3.5}
    %     \label{fig:REF_GPT35}
    % \end{subfigure}
     \caption{Trace complexity analysis for all dataset-model pairs given correct and incorrect programs.}
    \label{fig:tranly}
\end{figure}
%In this research question, our objective is to understand the effectiveness of few-shot (FS) and chain-of-thought (COT) prompts to improve the capability of GPT models in APR task.
 %We first discuss about both prompts and then discuss the evaluation results.








%%To understand the effectiveness of execution traces in GPT model for APR, we feed prompts to GPT models that have faulty program, assertion errors and execution traces in the prompt. We name these prompts as \textit{\textbf{Trace Prompts (TP)}}. Additionally, we use two different type of prompts as baseline to compare with prompt with execution traces.  For the first baseline, we additionally use assertion errors in the prompt other than the faulty program. These prompts are referred as \textit{\textbf{Error Prompts (EP)}}. For both EP and TP, we create multiple combination between unique faulty program from the dataset and corresponding unit test cases.In the second baseline, we do not provide any additional information other than the faulty program in the prompt. We refer these kind of prompts as \textit{\textbf{Vanilla Prompts (VP)}}. To limit the prompt size within the GPT model context-size, we limit the number of lines to 200, \textit{e.g.}, we remove the content of prompt if the line number is higher than 200.

%\subsection{RQ3.  Does any type of bugs specifically need the program-traces to be fixed?}
\begin{comment}
\begin{figure*}
\tiny

\begin{tikzpicture}[fill=gray]
% left hand
\scope
\clip (-2,-2) rectangle (2,2)
      (1,0) circle (1);
\fill (0,0) circle (1);
\endscope
% right hand
\scope
\clip (-2,-2) rectangle (2,2)
      (0,0) circle (1);
\fill (1,0) circle (1);
\endscope
% outline
\draw (0.35, 0) node [text=black,right] {37} % intersection
      (0,0) circle (1) (0,1)  node [text=black,above] {VP} node [text=black,below] {3} 
      (1,0) circle (1) (1,1)  node [text=black,above] {EP} node [text=black,below] {20} ;
\end{tikzpicture}



%%%%%%%%% FIRST ROW
\begin{multicols}{4}
\begin{tikzpicture}[fill=gray]
% left hand
\scope
\clip (-2,-2) rectangle (2,2)
      (1,0) circle (1);
\fill (0,0) circle (1);
\endscope
% right hand
\scope
\clip (-2,-2) rectangle (2,2)
      (0,0) circle (1);
\fill (1,0) circle (1);
\endscope
% outline
\draw (0.35, 0) node [text=black,right] {53} % intersection
      (0,0) circle (1) (0,1)  node [text=black,above] {EP} node [text=black,below] {4} 
      (1,0) circle (1) (1,1)  node [text=black,above] {TP} node [text=black,below] {5} ;
\end{tikzpicture}


\begin{tikzpicture}[fill=gray]
% left hand
\scope
\clip (-2,-2) rectangle (2,2)
      (1,0) circle (1);
\fill (0,0) circle (1);
\endscope
% right hand
\scope
\clip (-2,-2) rectangle (2,2)
      (0,0) circle (1);
\fill (1,0) circle (1);
\endscope
% outline
\draw (0.35, 0) node [text=black,right] {48} % intersection
      (0,0) circle (1) (0,1)  node [text=black,above] {EP} node [text=black,below] {9} 
      (1,0) circle (1) (1,1)  node [text=black,above] {FST} node [text=black,below] {3} ;
\end{tikzpicture}


\begin{tikzpicture}[fill=gray]
% left hand
\scope
\clip (-2,-2) rectangle (2,2)
      (1,0) circle (1);
\fill (0,0) circle (1);
\endscope
% right hand
\scope
\clip (-2,-2) rectangle (2,2)
      (0,0) circle (1);
\fill (1,0) circle (1);
\endscope
% outline
\draw (0.35, 0) node [text=black,right] {44} % intersection
      (0,0) circle (1) (0,1)  node [text=black,above] {EP} node [text=black,below] {13} 
      (1,0) circle (1) (1,1)  node [text=black,above] {COTT} node [text=black,below] {0} ;
\end{tikzpicture}



\begin{tikzpicture}[fill=gray]
% left hand
\scope
\clip (-2,-2) rectangle (2,2)
      (1,0) circle (1);
\fill (0,0) circle (1);
\endscope
% right hand
\scope
\clip (-2,-2) rectangle (2,2)
      (0,0) circle (1);
\fill (1,0) circle (1);
\endscope
% outline
\draw (0.35, 0) node [text=black,right] {38} % intersection
      (0,0) circle (1) (0,1)  node [text=black,above] {EP} node [text=black,below] {19} 
      (1,0) circle (1) (1,1)  node [text=black,above] {FST-Ext} node [text=black,below] {2} ;
\end{tikzpicture}
\end{multicols}






%%%%%%%%% SECOND ROW
\begin{multicols}{4}
\begin{tikzpicture}[fill=gray]
% left hand
\scope
\clip (-2,-2) rectangle (2,2)
      (1,0) circle (1);
\fill (0,0) circle (1);
\endscope
% right hand
\scope
\clip (-2,-2) rectangle (2,2)
      (0,0) circle (1);
\fill (1,0) circle (1);
\endscope
% outline
\draw (0.35, 0) node [text=black,right] {53} % intersection
      (0,0) circle (1) (0,1)  node [text=black,above] {FSE} node [text=black,below] {2} 
      (1,0) circle (1) (1,1)  node [text=black,above] {TP} node [text=black,below] {5} ;
\end{tikzpicture}






\begin{tikzpicture}[fill=gray]
% left hand
\scope
\clip (-2,-2) rectangle (2,2)
      (1,0) circle (1);
\fill (0,0) circle (1);
\endscope
% right hand
\scope
\clip (-2,-2) rectangle (2,2)
      (0,0) circle (1);
\fill (1,0) circle (1);
\endscope
% outline
\draw (0.35, 0) node [text=black,right] {50} % intersection
      (0,0) circle (1) (0,1)  node [text=black,above] {FSE} node [text=black,below] {5} 
      (1,0) circle (1) (1,1)  node [text=black,above] {FST} node [text=black,below] {1} ;
\end{tikzpicture}






\begin{tikzpicture}[fill=gray]
% left hand
\scope
\clip (-2,-2) rectangle (2,2)
      (1,0) circle (1);
\fill (0,0) circle (1);
\endscope
% right hand
\scope
\clip (-2,-2) rectangle (2,2)
      (0,0) circle (1);
\fill (1,0) circle (1);
\endscope
% outline
\draw (0.35, 0) node [text=black,right] {44} % intersection
      (0,0) circle (1) (0,1)  node [text=black,above] {FSE} node [text=black,below] {11} 
      (1,0) circle (1) (1,1)  node [text=black,above] {COTT} node [text=black,below] {0} ;
\end{tikzpicture}





\begin{tikzpicture}[fill=gray]
% left hand
\scope
\clip (-2,-2) rectangle (2,2)
      (1,0) circle (1);
\fill (0,0) circle (1);
\endscope
% right hand
\scope
\clip (-2,-2) rectangle (2,2)
      (0,0) circle (1);
\fill (1,0) circle (1);
\endscope
% outline
\draw (0.35, 0) node [text=black,right] {40} % intersection
      (0,0) circle (1) (0,1)  node [text=black,above] {FSE} node [text=black,below] {15} 
      (1,0) circle (1) (1,1)  node [text=black,above] {FST-Ext} node [text=black,below] {0} ;
\end{tikzpicture}


\end{multicols}

\end{figure*}
\end{comment}



\begin{comment}

\begin{figure*}
\begin{multicols}{3}
    


%%% FIRST ROW GPT4
\begin{tikzpicture}[fill=gray]
% left hand
\scope
\clip (-2,-2) rectangle (2,2)
      (1,0) circle (1);
\fill (0,0) circle (1);
\endscope
% right hand
\scope
\clip (-2,-2) rectangle (2,2)
      (0,0) circle (1);
\fill (1,0) circle (1);
\endscope
% outline
\draw (0.35, 0) node [text=black,right] {65} % intersection
      (0,0) circle (1) (0,1)  node [text=black,above] {EP} node [text=black,below] {1} 
      (1,0) circle (1) (1,1)  node [text=black,above] {TP} node [text=black,below] {0} ;
\end{tikzpicture}

\begin{tikzpicture}[fill=gray]
% left hand
\scope
\clip (-2,-2) rectangle (2,2)
      (1,0) circle (1);
\fill (0,0) circle (1);
\endscope
% right hand
\scope
\clip (-2,-2) rectangle (2,2)
      (0,0) circle (1);
\fill (1,0) circle (1);
\endscope
% outline
\draw (0.35, 0) node [text=black,right] {61} % intersection
      (0,0) circle (1) (0,1)  node [text=black,above] {EP} node [text=black,below] {5} 
      (1,0) circle (1) (1,1)  node [text=black,above] {FST} node [text=black,below] {0} ;
\end{tikzpicture}


\begin{tikzpicture}[fill=gray]
% left hand
\scope
\clip (-2,-2) rectangle (2,2)
      (1,0) circle (1);
\fill (0,0) circle (1);
\endscope
% right hand
\scope
\clip (-2,-2) rectangle (2,2)
      (0,0) circle (1);
\fill (1,0) circle (1);
\endscope
% outline
\draw (0.35, 0) node [text=black,right] {61} % intersection
      (0,0) circle (1) (0,1)  node [text=black,above] {EP} node [text=black,below] {5} 
      (1,0) circle (1) (1,1)  node [text=black,above] {COTT} node [text=black,below] {0} ;
\end{tikzpicture}

\end{multicols}





%%% SECOND ROW

\begin{multicols}{3}


    \begin{tikzpicture}[fill=gray]
% left hand
\scope
\clip (-2,-2) rectangle (2,2)
      (1,0) circle (1);
\fill (0,0) circle (1);
\endscope
% right hand
\scope
\clip (-2,-2) rectangle (2,2)
      (0,0) circle (1);
\fill (1,0) circle (1);
\endscope
% outline
\draw (0.35, 0) node [text=black,right] {64} % intersection
      (0,0) circle (1) (0,1)  node [text=black,above] {FSE} node [text=black,below] {1} 
      (1,0) circle (1) (1,1)  node [text=black,above] {TP} node [text=black,below] {1} ;
\end{tikzpicture}




\begin{tikzpicture}[fill=gray]
% left hand
\scope
\clip (-2,-2) rectangle (2,2)
      (1,0) circle (1);
\fill (0,0) circle (1);
\endscope
% right hand
\scope
\clip (-2,-2) rectangle (2,2)
      (0,0) circle (1);
\fill (1,0) circle (1);
\endscope
% outline
\draw (0.35, 0) node [text=black,right] {61} % intersection
      (0,0) circle (1) (0,1)  node [text=black,above] {FSE} node [text=black,below] {4} 
      (1,0) circle (1) (1,1)  node [text=black,above] {FST} node [text=black,below] {0} ;
\end{tikzpicture}


\begin{tikzpicture}[fill=gray]
% left hand
\scope
\clip (-2,-2) rectangle (2,2)
      (1,0) circle (1);
\fill (0,0) circle (1);
\endscope
% right hand
\scope
\clip (-2,-2) rectangle (2,2)
      (0,0) circle (1);
\fill (1,0) circle (1);
\endscope
% outline
\draw (0.35, 0) node [text=black,right] {61} % intersection
      (0,0) circle (1) (0,1)  node [text=black,above] {FSE} node [text=black,below] {4} 
      (1,0) circle (1) (1,1)  node [text=black,above] {COTT} node [text=black,below] {0} ;
\end{tikzpicture}


\end{multicols}

\caption{GPT 4 Refactory}
\end{figure*}

\end{comment}


 

Unlike other elements of the prompt, execution traces are dynamic in nature and are highly dependent on a particular input as much as the program itself. Additionally, execution traces can be dramatically different in the presence of a runtime error, compared to when the function finishes correctly (even if the returned value itself is wrong).
Thus variations in trace complexity could be a crucial factor of how beneficial their inclusion is in the prompt. On the one hand, traces that are too short may not provide much information beyond what is already conveyed by the program itself and the failing test case. On the other hand, overly long and complex traces may overwhelm LLMs long context and ultimately confuse it.
We believe there is a sweet spot at which the inclusion of traces is most beneficial.
As such, we observed great variability with respect to the overall trace length, as well as in the number and type of individual state changes. \todo{examples in appendix}

To gain insights into nuanced differences among our evaluated datasets, we compute the statistics of overall trace length and the number of variable modifications in all prompts, while differentiating by whether the resulting fix was correct. 
For both the HumanEval-Java and RunBugRun datasets median\footnote{In all datasets and for both correct and failing fixes we observed the presence of extremely long traces in excess of 10,000 entries. Additionally, a significant number of trace prompts got truncated (5\% for Refactory and almost 10\% for run\_bug\_run). %Truncation has multiple implications for performance: firstly, information contained in the prompt is partial; secondly it is an indirect indication of potentially overwhelming the LLMs ability to deal with long context. \todo{run with 16k context}
} trace length and number of variable modifications were significantly higher for failing fixes than for the correct ones. This corroborates our presupposition that longer traces could undermine rather than help APR. 
Conversely, in the Refactory dataset, somewhat contrary to our intuitions, for failing fixes median trace length were actually lower than for successful fixes. When it comes to the number of variable modifications, the median was just one, compared to 5 in RunBugRun. This disparity implies variable modifications could play a key role in the effectiveness of a trace for APR.



% \todo{complexity analysis} \todo{probing study}



% In this research question, we discuss if any type of bug can be solved exclusively when using execution traces. In the previous sections, we find that adding execution traces does not provide any guarantee for improving the program repair capability in the models. However, it is important to understand if any specific bugs are only solved using trace-based prompts. For that purpose, we compare programs fixed by different error-based and trace-based prompts and produce Venn diagram that can show the number of faulty programs fixed by only that prompt type. However, our main objective is to analyze the Venn diagrams between EP-TP and FSE-FST across different datasets and GPT. 

% Figure \ref{fig:rq3_java_gpt3.5}, \ref{fig:rq3_py_gpt3.5}, \ref{fig:rq3_java_gpt4} and \ref{fig:rq3_py_gpt4} show our findings (Last three figures are in appendix). For HumanEval-Java dataset, it is evident that trace-based programs fix a significant number of faulty programs that are not solved by error-based prompts. Specifically, TP always solves more number of unique programs than EP.


% %for GPT-4 model, the numbers are higher. For example, for GPT-4 model, FSE and TP prompts both help to fix 112 programs; however, 17 of the faulty programs are only solved by FSE or TP prompts. 

% On the contrary, for Refactory dataset, few programs are only solved by trace-based prompts. These results further support the claim that GPT models can not utilize the execution traces to fix programs in the Refractory dataset.  

 
\begin{center}
\begin{tcolorbox}[colback=gray!10,%gray background
                  colframe=black,% black frame colour
                  width=7.5cm,% Use 8cm total width,
                  arc=1mm, auto outer arc,
                  boxrule=0.9pt,
                 ]
 \textbf{RQ2 Summary.} The prompts having longer execution traces have a lesser chance of repairing a faulty program. 
\end{tcolorbox}
\end{center}

\subsection{RQ3. How do modified traces perform against library-generated execution traces for repairing programs?}
\todo[author=Petr]{Add the modified RQ3 here.}

\subsection{Collated Execution Traces}

Even though execution traces for both languages reference code lines from the original program, they are placed in the standalone section of the prompt, separate from the program itself.
In order to thoroughly ablate trace format we experimented with combining the two by placing each trace entry directly to its corresponding line of code as an inline comment \footnote{In case of multiple passes through the same line e.g., varible changes within a loop, we concatenate each of the traced events by a new line, providing a full history of state changes at that line.}. The rationale behind this design choice is to consolidate the two types of information in the common location, potentially freeing the LLM from having to constantly cross-reference between them. 

\subsection{LLM-Summarized Execution Traces}
%\todo[author=Miraz]{Add the Summarized traces details here.}
LLM-summarized execution traces are condensed versions of deterministic traces. While deterministic traces provide notable information regarding variable changes, in multiple scenarios, they can also be lengthy. For example, if a loop counter is stuck in an infinite loop, it will add numerous number of lines to the deterministic execution traces. This would not increase the trace length without adding significant valuable information. A summarized version of these traces might be more helpful for GPT models in understanding the faulty program.

To generate summarized execution traces, we use GPT4-32k model. The deterministic execution trace is sent to the model and prompted to generate a summarized version of the trace.

\subsection{Conditionally Selected Execution Traces}
In this particular approach, we do not generate any new type of execution traces, but we prompt GPT models to select if the model is confident about using deterministic traces to repair the program. If the confidence level is low, an LLM-summarized trace will be used.

We have considered multiple ways to find the confidence value of the model. One possible way is to prompt the model to find whether it's confident or not (boolean) to use a specific prompt to repair a program. But on a small prompt set, we find that the model outputs that it is always confident for all inputs. Additionally, another way is to feed both prompts and ask the model for which prompt it is more confident to repair the program. However, based on the findings of recent work~\cite{huang2023embrace}, LLM might be biased for a specific position (prompt one or prompt two). Hence, based on the findings of Huang et al.~\cite{huang2023embrace}, we use a likert-scale based confidence score. Given a score range of 1-5, if the confidence score provided by the model is less than 3, we consider that the model has low-confidence. The approach is shown in Figure \ref{fig:cond}.


To ensure the prompt and response fit within the GPT model context size, we truncate the content of the prompt if the number of lines exceeds 200.
All the used prompts can be found at: https://anonymous.4open.science/r/CodePlanGPT-DBF3/. Additionally, we have added an example of all the prompts in Section \ref{sec:prompt} in the Appendix.


%\todo[author=Miraz]{Add the Conditional traces details here.}
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[h!]
\centering
\caption{Quantitative Results for RQ3. Bold indicates configurations outperforming the best configuration from RQ1 for a given model and dataset. Italic indicates parity with the best configuration from RQ1.}
\begin{tabular}{lllrrrr}
Dataset   Name                   & Prompt Type                            & Model                         & \textbf{\#FP}           & \textbf{\#Fixes}        & \textbf{CFA}                 & \textbf{CPA}                 \\ \hline
\multirow{6}[1]{*}{Refactory}                        & Collated Trace                         & \multirow{3}[1]{*}{GPT3.5}                       & 136                     & 561                     & 0.467023                     & 0.595588                     \\
                        & OPT Prompt                             &                        & 136                     & 563                     & 0.516874                     & 0.610294                     \\
 & Conf OPT Prompt & &  &  &       &       \\

\cline{2-7}
                        & Collated Trace                         & \multirow{3}[1]{*}{GPT4}                        & 136 & 563 & 0.674956 & 0.830882 \\
                        & OPT Prompt                             &                           & 137                     & 565                     & 0.771681                     & 0.868613                     \\
                        & Conf OPT Prompt                        &                           & 136                     & 561                     & 0.759358                     & 0.860294                     \\
\hline
\multirow{6}[1]{*}{HEJ}       & Collated Trace  & \multirow{3}[1]{*}{GPT3.5} &  &  &       &       \\
                              & OPT Prompt                             &                      & 157                     & 634                     & \textbf{0.430599}                    & 0.535032                     \\
                              & Conf OPT Prompt                        &                         & 157                     & 634                     & 0.380126                     & 0.522293                     \\
\cline{2-7}
       & Collated Trace  &  \multirow{3}[1]{*}{GPT4}   &   &  &  &      \\
                              & OPT Prompt                             &                           & 157                     & 634                     & \textbf{0.572555}                     & \textit{0.713376}                    \\
                              & Conf OPT Prompt                        &                           & 157                     & 634                     & 0.548896                     & \textbf{0.732484}                     \\
\hline
\multirow{6}[1]{*}{rbugr}                           & Collated Trace                         & \multirow{3}[1]{*}{GPT3.5}                   & 439                     & 534                     & 0.398876                     & 0.42369                      \\
                            & OPT Prompt                             &                         & 453                     & 555                     & \textbf{0.475676}                     & \textbf{0.501104}                     \\
                            & Conf OPT Prompt                        &                         & 456                     & 559                     & 0.429338                     & 0.453947                     \\
\cline{2-7}
                            & Collated Trace                         & \multirow{3}[1]{*}{GPT4}                          & 439                     & 533                     & 0.506567                     & 0.528474                     \\
                            & OPT Prompt                             &                           & 452                     & 555                     & \textbf{0.574775}                     & \textbf{0.595133}                     \\
                            & Conf OPT Prompt                        &                           & 456                     & 559                     & 0.527728                     & 0.550439        \\ \hline            
\end{tabular}
\end{table*}
In this RQ, we discuss the impact of modified DTP-based approaches on program repair. As in RQ2, we could find that trace complexity can be correlated with the APR capability; we consider the following three prompting techniques for program repair: Collated Trace Prompts (CTP), Summarized Trace Prompts (STP), and Conditional Selection of Traces (CST).  

%We consider three techniques her 



The results could be founding Table \ref{tab:addlabel_2}. Disappointingly, CTP does not provide an improvement over DTP. One possible explanation is a lack of exposure to this format during LLM training as code doesn't normally include inline comments about state changes.
Second, inline traces within loops can ``stretch'' the length of the program quite a bit, possibly diluting LLMs attention to the continuation of the program after the loop. In our probing studies of LLM trace understanding we find that indeed LLMs struggle keeping up with variable changes across multiple-iterations. Lastly, the problem of truncation becomes more severe with collated traces as not just the trace but also part of the original problem could be excluded from the prompt as a result.

STP is the most consistently performing prompting technique, considering both CFA and CPA. With respect to CPA, for all dataset and model pairs, STP is among the top three performing prompting techniques. The CFA values for STP are even more commendable, where for four out of six model-dataset pairs STP has the best CFA (second best in the other two). Furthermore, this confirms our implication from RQ2 that less complicated traces are better for prompting for program repair tasks. 

For CST, while we find the CFA and CPA values are comparatively better for GPT4, the performance in GPT3.5 is worse. This would imply that GPT-4 is significantly better in providing confidence scores for prompts than GPT-3.5. But, as the performance is significantly worse than STP on average, the application of the method for GPT-4 is still not reliable. 


%\def\cca#1{\cellcolor{black!#10}\ifnum #1>5\color{white}\fi{#1}}
%In this section, we discuss different types of bugs present in the unique faulty programs repaired by error-based (EP, FSE) and trace-based prompts (TP, FST). Table \ref{tab:RQ3} shows our results. The error types mentioned in the table are operations that must be performed on the faulty program to get the correct program based on the taxonomy introduced in HumanEval-Java. For each row, the term $X>Y$ focuses on the error types in the programs repaired by the specific type of prompt $X$, but not repaired by the prompt type $Y$.

%For the HumanEval-Java dataset on GPT-4, we could find that more errors belonging to error types like Conditional Branch Addition and Method Call Parameter Modification have been solved uniquely by TP against EP. Additionally, Method Call Addition error types have been solved uniquely by FST against FSE. However, for the HumanEval-Java dataset on GPT-3.5, we do not find a similar pattern. TP could repair more number of errors belong to error types like Return Expression Modification and Variable Modification (against EP). On the other hand, FST could solve more errors belonging to Initialization Modification, Loop Condition Modification, and Type Modification.

%Unlike HumanEval-Java, Refactory does not include annotations of bug types present in a given faulty program. Thus, we had to manually classify bug types by analyzing the diffs to the closest working program by edit distance. Consequently, for only half of the considered Refactory programs bug types could be clearly identified. The reason is most of the faulty programs from this dataset have logical flaws not localized to particular statements and need extensive modification to obtain the correct solution. Among the analyzed programs, we find error types related to method calls are solved more frequently by TP with GPT-3.5.
%, and Method Call Addition have been solved uniquely by TP and FST against EP and FSE, respectively.

%have been used to induce fault in HumanEval-Java dataset.  

\begin{center}
\begin{tcolorbox}[colback=gray!10,%gray background
                  colframe=black,% black frame colour
                  width=7.5cm,% Use 8cm total width,
                  arc=1mm, auto outer arc,
                  boxrule=0.9pt,
                 ]
 \textbf{RQ3 Summary.} Summarized Trace Prompt is the most consistent type of prompting technique, specifically for CFA metric.
\end{tcolorbox}
\end{center}

\subsection{ Is fine-tuning a better option than prompting for program repair?}

In this RQ, we focus on evaluating if fine-tuning a small-sized LLM would generate better results w.r.t program repair rather than prompting GPT models with different prompts. For that purpose, we fine-tune the deepseek-coder-1.3b-instruct model with training data extracted from HumanEval-Java and RunBugRun dataset. Finally, we compare the program repair performance of fine-tuning and prompting-based techniques on test data.

Table \ref{tab:ft} shows the results. It can be noted that all the prompting techniques outperform fine-tuned model's CPA and CFA. 

\begin{table*}[h!]
\centering
\caption{\textbf{CPA and CFA of prompting-based techniques with comparison to model fine-tuned for APR tasks.}}
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{c|c c|c c|c c|c c|c c|c c}
\hline
 Datasets& \multicolumn{2}{c|}{FT} & \multicolumn{2}{c|}{EP} & \multicolumn{2}{c|}{DTP} & \multicolumn{2}{c|}{CTP} & \multicolumn{2}{c|}{STP} & \multicolumn{2}{c}{CST} \\
 & CFA & CPA & CFA & CPA & CFA & CPA & CFA & CPA & CFA & CPA & CFA & CPA \\
\hline
Refactory &  &  &  &  &  &  &  &  &  &  &  &  \\
HEJ       & 0.215 & 0.206 & 0.494 & 0.689  &0.505  & 0.724 & 0.613 &0.758  & 0.645 & 0.758 &0.602  & 0.827 \\
RBugR     &  &  &  &  &  &  &  &  &  &  &  &  \\

\hline
\end{tabular}}

\label{tab:ft}
\end{table*}

==> sections/evaluation_old.tex <==
\label{sec:eval}
We aim to answer three research question with our evaluation.

\noindent\textbf{RQ1.} Can execution traces in the prompt help the LLMs fix an incorrect program?

\noindent\textbf{RQ2.} Are any bugs uniquely solved by including program execution traces in the prompt?



\noindent\textbf{RQ3.} Which types of bugs require  specifically program execution traces in order to be fixed?
\subsection{Set Up}
\noindent\textbf{Datasets.} For our experiments, we used two recent APR datasets: Refactory~\cite{hu2019re}, RunBugRun(Python data)~\cite{} and Humaneval-Java~\cite{jiang2023impact}. Refractory consists of faulty Python programs submitted by students, whereas the 

HumanEval-Java dataset is created by introducing bugs to the HumanEval dataset. Manually created datasets like HumanEval-Java help to create a diversity among the errors present in the faulty program. These two datasets would highlight GPT model's ability to reason about program execution across different languages. 

\noindent\textbf{Models.} We use two state-of-the-art GPT models for evaluation: GPT-4~\cite{OpenAI2023GPT4TR} and GPT-3.5 Turbo ~\cite{ouyang2022training}. These two models are different w.r.t number of parameters, hence, selecting these models for evaluation can provide an understanding about GPT model's ability to reason about program execution with different number of parameters.

\noindent\textbf{Prompt Types.} To understand the effectiveness of execution traces in the GPT model for APR, we feed various prompts (including and excluding execution traces) to GPT models. First type of prompts are called \textit{\textbf{Program Prompts (PP)}}, in which the faulty program is fed to the GPT models without any additional details. in the second type of prompts, we include test case assertion errors in the prompt together with the faulty program (\textbf{PP+Error} ). These prompts are called \textit{\textbf{Error Prompts (EP)}}. Third type of prompts are called \textit{\textbf{Trace Prompts (TP)}}, where we include execution trace along with faulty program and assertion error in the prompt (\textbf{PP+Error+Trace}). 

To improve the prompt effectiveness, we use few-shot (FS) prompts with both errors and traces. These prompts are called few-shot error (FSE) prompts and few-shot trace (FST) prompts. In these prompts, we first randomly select five examples from the dataset and randomly use three of the examples in the prompt. For FSE, the examples include faulty program, assertion error and correct program. While for FST, the examples also include execution traces (\textbf{FSE+Trace}). 

Each of the prompts only includes a single program with a single test case. Although we understand that having multiple test-cases in a single program can have a better possibility in repairing a program, our objective in the work is to find the effect of adding execution traces to the prompt. Hence, we only create prompts where we can show the evaluation with both including and excluding traces. If we were to use multiple test cases in a prompt, that might lead to having multiple execution traces in the prompt, which can lead to prompts exceeding maximum context length.  

Additionally, we use enriched prompts like chain-of-thought prompting  with traces (COTT) and extended few shot prompts with traces (FST-Ext) to measure if enriched prompts can improve the program repairing capability of trace prompts or not. For COTT, we modify the instruction in the FST prompts to first find the location of the bug rather than provide a fix in one shot. The response to that prompt is then chained with the instruction to provide a fix based on the bug location predicted at the previous step. For FST-Ext, we extend the few-shot examples to include the trace of the correct program execution in addition to the failing one.


%For chain-of-thought prompting (COTT), we modify the instruction in the FST prompts to first find the location of the bug rather than provide a fix on one shot. The response to that prompt is then chained with the instruction to provide a fix based on the bug location predicted at the previous step.

%Additionally, we use extended few shot prompts with traces (FST-Ext), which extends the few-shot examples to include the trace of the correct program execution in addition to the failing one. The intuition behind using the correct trace is that GPT model might be able to understand the failing execution traces better if both correct and wrong traces are provided in the example. 
We follow prompt format from Xia et al. (~\citeyear{ICSE10172803}).
To ensure the prompt and response fit within the GPT model context-size, we truncate the content of the prompt if the number of lines exceeds 200 (For TP, EP and PP).
However, for the FS prompts, instead of removing prompt content abruptly, we try to modify the number of few-shot examples in the prompt. While iteratively adding the examples to the prompt, if addition of an example in the prompt leads to crossing the line limit, that few-shot example is not added. All the used prompts can be found at: https://anonymous.4open.science/r/CodePlanGPT-DBF3/. Additionally, I have added an example of EP, TP, FSE, and FST prompts in Section \ref{sec:prompt} in the Appendix.








%that have faulty program, assertion errors, and execution traces in the prompt. We name these prompts as \textit{\textbf{Trace Prompts (TP)}}. Additionally, we use two different types of prompts as baselines to compare prompts with execution traces.  For the first baseline, we include test case assertion errors in the prompt together with the faulty program but not the execution trace. These prompts are referred to as \textit{\textbf{Error Prompts (EP)}}. For both EP and TP, we create multiple combinations between unique faulty programs from the dataset and corresponding unit test cases.In the second baseline, we do not provide any additional information other than the faulty program in the prompt. We refer these kind of prompts as \textit{\textbf{Program Prompts (PP)}}. 


\noindent\textbf{Metric.} 
In previous work on APR, models are evaluated either at the granularity of distinct bugs solved cf. -- \cite{ICSE10172803}, \cite{jiang2023impact} or individual test cases passed \cite{tian2023chatgpt}.
In both cases, the model is prompted once with each buggy program, and results are aggregated from multiple output samples from the APR model.
In our case, we obtain multiple prompts for a given program -- each one specific to a particular failing test case and the corresponding execution trace.
Rather than aggregating from multiple sampled predictions, we obtain a single prediction for each test case-specific prompt and aggregate them across prompts when computing the metrics.%, while setting the GPT model's temperature parameter to 0. 
To make our results comparable to previous work, we report accuracy at the level of individual test cases, generated fixes, and finally unique buggy programs.
% We use three metrics to explore the GPT model's capability to reason about execution traces. 
\textit{\textbf{Correct Test Accuracy (CTA)}} evaluates the percentage of unit test cases that are correct using at least one of the GPT-generated fixes.
%We report accuracy of the LLM using two metrics. 
\textit{\textbf{Correct Fix Accuracy (CFA)}} evaluates the percentage of correct fixes generated by GPT model given a specific type of prompt. \textit{\textbf{Correct Program Accuracy (CPA)}} evaluates the percentage of faulty programs solved by GPT model given a specific type of prompt. 

To illustrate, let's assume the dataset has 10 faulty programs, each with 5 unit test cases (50 unique test cases). For Error Prompts (EP) and Trace Prompts (TP), 50 different prompts are created, which are fed to a GPT model. GPT model would generate 50 corresponding program fixes. Those 50 program fixes are evaluated on 5 unit test cases. If 25 of the 50 unique test cases are passed by at least one fix, then CTA would be (25/50)*100=50\%. If out of 50 program fixes, 10 programs pass all 5 test cases, the CFA would be (10/50)*100=25\%. Also, if there are five programs out of 10 faulty programs for which at least one program is generated that passes all unit test cases, then CPA would be (5/10)*100=50\%.

\begin{figure*}[!t]
    \centering
\begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{figures/GPT35_HEJ.pdf}
        \caption{HumanEval-Java Dataset with GPT-3.5 }
         \label{fig:HEJ_GPT35}
    \end{subfigure}
    % \begin{subfigure}[b]{0.355\textwidth}
    %     \includegraphics[width=\textwidth]{figures/corruption_skipnet.pdf}
    %     \caption{Effect of corruption on SkipNet}
    % \end{subfigure}
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{figures/GPT4_HEJ.pdf}
        \caption{HumanEval-Java Dataset with GPT-4}
        \label{fig:HEJ_GPT4}
    \end{subfigure}

    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{figures/GPT35_REF.pdf}
        \caption{Refactory Dataset with GPT-3.5 }
         \label{fig:REF_GPT35}
    \end{subfigure}
    % \begin{subfigure}[b]{0.355\textwidth}
    %     \includegraphics[width=\textwidth]{figures/corruption_skipnet.pdf}
    %     \caption{Effect of corruption on SkipNet}
    % \end{subfigure}
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{figures/GPT4_REF.pdf}
        \caption{Refactory Dataset with GPT-4}
        \label{fig:REF_GPT4}
    \end{subfigure}
     \caption{CPA, CFA, and CTA values for different prompts. 'CPA', 'CFA', and  'CTA' are represented by  'skyblue',  'lightgreen',  'salmon' color bars respectively.}
    \label{fig:acc}
\end{figure*}

All three metrics have significance in quantifying GPT model's capability for program repair. CTA would compare whether every failing test case received at least one working fix. However, CTA is not able to measure how many of the generated fixes are fully correct (Having CTA of 50\% does not guarantee 50\% correct programs). Hence, the usage of CFA is important. Also, it is possible that GPT model is generating multiple correct fixes for one faulty program, while for other faulty programs, none of the generated fixes are correct. Hence, CPA measurement also becomes important.
\begin{figure*}
  \begin{center}
    \includegraphics[width=0.8\textwidth]{figures/Findings-GPT3.5.drawio-2.pdf}
  \end{center}
  \caption{Venn diagrams showing fixed programs which are solved only using different error-based and trace-based prompts (For GPT-3.5 model and HumanEval-Java dataset.)}
  \label{fig:rq3_java_gpt3.5}
\end{figure*}
\subsection{RQ1. Can execution trace in prompt help GPT models to fix an incorrect program?}
 \begin{comment}
     \multirow{1}[2]{*}{Model} & \multirow{1}[2]{*}{Dataset} & \multicolumn{1}{c|}{\multirow{1}[2]{*}{Prompt Type}} & \multicolumn{1}{c|}{# of Faulty Programs} & \multicolumn{1}{c|}{# of Prompts} & \multicolumn{1}{c|}{# of Test Cases} & \multicolumn{1}{c|}{# of Correct Programs} & \multicolumn{1}{c|}{# of Correct Unique Programs} & \multicolumn{1}{c}{# of Correct Test Cases} &  \multicolumn{1}{c}{CTA}&  \multicolumn{1}{c}{CPA} & \multicolumn{1}{c}{CUPA}\\
 \end{comment}



In this research question, our objective is to compare the effectiveness of GPT model against APR tasks with and without execution traces in the prompt. To evaluate the effectiveness, we use three metrics (CPA, CFA, and CTA) on the responses generated by aforementioned prompts. The objective is to determine the effectiveness of added traces in the prompts. Hence, we mainly compare PP-EP-TP and FSE-FST results. 

%We first discuss about different used prompt-types and then discuss the evaluation results.


%We have used multiple types of prompts for TP and EP, which are discussed in details during exploring the RQs.

\noindent\textbf{Evaluation Results.} The evaluation results can be found in Figure \ref{fig:acc} (The full results can be found in Table \ref{tab:addlabel}). The number of faulty programs and total test cases is the same for all types of prompts per each dataset, while the number of fixes is the same for all types of prompts except PP (as PP does not include any test cases).   

For HumanEva-Java dataset, for both GPT-3.5 and GPT-4, TP-generated responses have higher CPA and CTA than PP and EP generated responses; showing that more faulty programs can be fixed if traces are added. However, in comparison between FSE and FST generated responses, we could find that adding few-shot examples can improve the error-based prompts significantly. However, adding few-shot examples to trace-based prompts could create large prompts, which can lead to a generation of more unusable responses (dropping the CPA). Also, using COTT and FST-Ext does not help trace-based prompts significantly, as this leads to larger prompts and more unusable responses.

One interesting observation is that having a higher CFA does not always lead to a higher CPA. These results indicate that a type of prompt could generate multiple correct fixes for one faulty program, showing higher CFA but lower CPA.

For the Refractory dataset, for the GPT-3.5 model, TP-generated responses repair a higher number of faulty programs than EP-generated responses; however, for GPT-4, the numbers remain the same. Similar to the findings for the HumanEval-Java dataset, for Refractory also, FST prompts fail to improve CPA more than FSE prompts.

%The first notable observation is that the number of faulty programs is not the same for all types of prompts. This is because of some of the responses generated by GPT model did not contain a valid fix and were thus discarded as unusable.

%For GPT-3.5 model and Refactory dataset, program prompt (PP) can generate 40 correct fixes that repair 40 programs. However, using error prompt (EP) or trace prompt (TP) improves the program repairing capability of GPT-3.5 significantly --- with more than double the CFA and CPA rates. With respect to CFA, EP performs approximately 3\% better than TP. However, w.r.t CPA, TP can generate more correct programs than PP and EP. The results indicate that EP could generate multiple correct fixes for one faulty program, but EP and TP's capability to generate fixes for different faulty programs is similar.




%For GPT-3.5 model and HumanEval-Java dataset, program prompt (PP) can not generate any correct fixes, surprisingly. However, using EP and TP significantly improves the capability of the GPT model. While CTA for TP is higher than EP, the CFA for EP is higher than TP. However, having a better percentage of correct fixes does not lead to having a better percentage of correct programs (CPA). TP helps to fix one program more than EP, given same number of faulty programs. Based on the results of both datasets, it is evident that execution traces do not help to improve GPT-3.5 in repairing programs. 



%For GPT-4 model, we could find different trends in our findings. For Refactory dataset, TP has lower effectiveness than EP w.r.t CTA and CPA. However, for HumanEval-Java dataset, TP performs extensively well by improving program repairing capability in GPT-4. TP could repair 112 programs (8 higher than EP generated correct programs) with a CPA of 72.2\%. These results suggest that for HumanEval-Java dataset, GPT-4 potentially relied on program execution traces to repair programs. One reason behind these contrastive results might be because of the formation of both datasets. Refactory is collected based on wrong programming assignment answers where the bug in the program might not be understood correctly with execution traces (\textit{e.g.,} missing return statement). While, the HumanEval-Java dataset is created by modifying existing lines of a correct program, where execution traces can provide a better idea of the bug.
\begin{center}
\begin{tcolorbox}[colback=gray!10,%gray background
                  colframe=black,% black frame colour
                  width=7.5cm,% Use 8cm total width,
                  arc=1mm, auto outer arc,
                  boxrule=0.9pt,
                 ]
 \textbf{RQ1 Summary.} Adding traces to prompts might be beneficial if the prompt size is not long.
\end{tcolorbox}
\end{center}


%\subsubsection{Set Up}


%\noindent\textbf{Evaluation Results.} The evaluation results can be found in Table \ref{tab:addlabel}. For Refactory dataset, few-shot examples do not improve the performance of GPT model for neither GPT-3.5 nor GPT-4 models (For both EP and TP). However FSE and FST prompts do not decrease the GPT model's program repairing capability either. By contrast, for the HumanEval-Java dataset, for both EP and TP, the program repair capability of GPT models increases significantly. 

%On the other hand, using chain-of-thought (COTT) and extended traces (FST-Ext) do not improve the program repairing capability of GPT model's on any datasets. For GPT-3.5 model, we could find significant drop in CPA by using COTT and FST-Ext prompts. For FST-Ext prompts, one of the reasons behind these results is because of longer few-shot prompt examples. Because of longer few-shot prompt examples, fewer examples could be added to the prompt, decreasing the few-shot capability.

\begin{comment}
\begin{center}
\begin{tcolorbox}[colback=gray!10,%gray background
                  colframe=black,% black frame colour
                  width=7.5cm,% Use 8cm total width,
                  arc=1mm, auto outer arc,
                  boxrule=0.9pt,
                 ]
 \textbf{RQ2 Summary.} Adding Few-shot examples do not improve the model's capability to repair programs always. Also, chain-of-thought prompting does not help in improving model capability.
\end{tcolorbox}
\end{center}
\end{comment}
\subsection{RQ2. Are any bugs uniquely solved by including program execution traces in the prompt?}

%In this research question, our objective is to understand the effectiveness of few-shot (FS) and chain-of-thought (COT) prompts to improve the capability of GPT models in APR task.
 %We first discuss about both prompts and then discuss the evaluation results.








%%To understand the effectiveness of execution traces in GPT model for APR, we feed prompts to GPT models that have faulty program, assertion errors and execution traces in the prompt. We name these prompts as \textit{\textbf{Trace Prompts (TP)}}. Additionally, we use two different type of prompts as baseline to compare with prompt with execution traces.  For the first baseline, we additionally use assertion errors in the prompt other than the faulty program. These prompts are referred as \textit{\textbf{Error Prompts (EP)}}. For both EP and TP, we create multiple combination between unique faulty program from the dataset and corresponding unit test cases.In the second baseline, we do not provide any additional information other than the faulty program in the prompt. We refer these kind of prompts as \textit{\textbf{Vanilla Prompts (VP)}}. To limit the prompt size within the GPT model context-size, we limit the number of lines to 200, \textit{e.g.}, we remove the content of prompt if the line number is higher than 200.

%\subsection{RQ3.  Does any type of bugs specifically need the program-traces to be fixed?}
\begin{comment}
\begin{figure*}
\tiny

\begin{tikzpicture}[fill=gray]
% left hand
\scope
\clip (-2,-2) rectangle (2,2)
      (1,0) circle (1);
\fill (0,0) circle (1);
\endscope
% right hand
\scope
\clip (-2,-2) rectangle (2,2)
      (0,0) circle (1);
\fill (1,0) circle (1);
\endscope
% outline
\draw (0.35, 0) node [text=black,right] {37} % intersection
      (0,0) circle (1) (0,1)  node [text=black,above] {VP} node [text=black,below] {3} 
      (1,0) circle (1) (1,1)  node [text=black,above] {EP} node [text=black,below] {20} ;
\end{tikzpicture}



%%%%%%%%% FIRST ROW
\begin{multicols}{4}
\begin{tikzpicture}[fill=gray]
% left hand
\scope
\clip (-2,-2) rectangle (2,2)
      (1,0) circle (1);
\fill (0,0) circle (1);
\endscope
% right hand
\scope
\clip (-2,-2) rectangle (2,2)
      (0,0) circle (1);
\fill (1,0) circle (1);
\endscope
% outline
\draw (0.35, 0) node [text=black,right] {53} % intersection
      (0,0) circle (1) (0,1)  node [text=black,above] {EP} node [text=black,below] {4} 
      (1,0) circle (1) (1,1)  node [text=black,above] {TP} node [text=black,below] {5} ;
\end{tikzpicture}


\begin{tikzpicture}[fill=gray]
% left hand
\scope
\clip (-2,-2) rectangle (2,2)
      (1,0) circle (1);
\fill (0,0) circle (1);
\endscope
% right hand
\scope
\clip (-2,-2) rectangle (2,2)
      (0,0) circle (1);
\fill (1,0) circle (1);
\endscope
% outline
\draw (0.35, 0) node [text=black,right] {48} % intersection
      (0,0) circle (1) (0,1)  node [text=black,above] {EP} node [text=black,below] {9} 
      (1,0) circle (1) (1,1)  node [text=black,above] {FST} node [text=black,below] {3} ;
\end{tikzpicture}


\begin{tikzpicture}[fill=gray]
% left hand
\scope
\clip (-2,-2) rectangle (2,2)
      (1,0) circle (1);
\fill (0,0) circle (1);
\endscope
% right hand
\scope
\clip (-2,-2) rectangle (2,2)
      (0,0) circle (1);
\fill (1,0) circle (1);
\endscope
% outline
\draw (0.35, 0) node [text=black,right] {44} % intersection
      (0,0) circle (1) (0,1)  node [text=black,above] {EP} node [text=black,below] {13} 
      (1,0) circle (1) (1,1)  node [text=black,above] {COTT} node [text=black,below] {0} ;
\end{tikzpicture}



\begin{tikzpicture}[fill=gray]
% left hand
\scope
\clip (-2,-2) rectangle (2,2)
      (1,0) circle (1);
\fill (0,0) circle (1);
\endscope
% right hand
\scope
\clip (-2,-2) rectangle (2,2)
      (0,0) circle (1);
\fill (1,0) circle (1);
\endscope
% outline
\draw (0.35, 0) node [text=black,right] {38} % intersection
      (0,0) circle (1) (0,1)  node [text=black,above] {EP} node [text=black,below] {19} 
      (1,0) circle (1) (1,1)  node [text=black,above] {FST-Ext} node [text=black,below] {2} ;
\end{tikzpicture}
\end{multicols}






%%%%%%%%% SECOND ROW
\begin{multicols}{4}
\begin{tikzpicture}[fill=gray]
% left hand
\scope
\clip (-2,-2) rectangle (2,2)
      (1,0) circle (1);
\fill (0,0) circle (1);
\endscope
% right hand
\scope
\clip (-2,-2) rectangle (2,2)
      (0,0) circle (1);
\fill (1,0) circle (1);
\endscope
% outline
\draw (0.35, 0) node [text=black,right] {53} % intersection
      (0,0) circle (1) (0,1)  node [text=black,above] {FSE} node [text=black,below] {2} 
      (1,0) circle (1) (1,1)  node [text=black,above] {TP} node [text=black,below] {5} ;
\end{tikzpicture}






\begin{tikzpicture}[fill=gray]
% left hand
\scope
\clip (-2,-2) rectangle (2,2)
      (1,0) circle (1);
\fill (0,0) circle (1);
\endscope
% right hand
\scope
\clip (-2,-2) rectangle (2,2)
      (0,0) circle (1);
\fill (1,0) circle (1);
\endscope
% outline
\draw (0.35, 0) node [text=black,right] {50} % intersection
      (0,0) circle (1) (0,1)  node [text=black,above] {FSE} node [text=black,below] {5} 
      (1,0) circle (1) (1,1)  node [text=black,above] {FST} node [text=black,below] {1} ;
\end{tikzpicture}






\begin{tikzpicture}[fill=gray]
% left hand
\scope
\clip (-2,-2) rectangle (2,2)
      (1,0) circle (1);
\fill (0,0) circle (1);
\endscope
% right hand
\scope
\clip (-2,-2) rectangle (2,2)
      (0,0) circle (1);
\fill (1,0) circle (1);
\endscope
% outline
\draw (0.35, 0) node [text=black,right] {44} % intersection
      (0,0) circle (1) (0,1)  node [text=black,above] {FSE} node [text=black,below] {11} 
      (1,0) circle (1) (1,1)  node [text=black,above] {COTT} node [text=black,below] {0} ;
\end{tikzpicture}





\begin{tikzpicture}[fill=gray]
% left hand
\scope
\clip (-2,-2) rectangle (2,2)
      (1,0) circle (1);
\fill (0,0) circle (1);
\endscope
% right hand
\scope
\clip (-2,-2) rectangle (2,2)
      (0,0) circle (1);
\fill (1,0) circle (1);
\endscope
% outline
\draw (0.35, 0) node [text=black,right] {40} % intersection
      (0,0) circle (1) (0,1)  node [text=black,above] {FSE} node [text=black,below] {15} 
      (1,0) circle (1) (1,1)  node [text=black,above] {FST-Ext} node [text=black,below] {0} ;
\end{tikzpicture}


\end{multicols}

\end{figure*}
\end{comment}



\begin{comment}

\begin{figure*}
\begin{multicols}{3}
    


%%% FIRST ROW GPT4
\begin{tikzpicture}[fill=gray]
% left hand
\scope
\clip (-2,-2) rectangle (2,2)
      (1,0) circle (1);
\fill (0,0) circle (1);
\endscope
% right hand
\scope
\clip (-2,-2) rectangle (2,2)
      (0,0) circle (1);
\fill (1,0) circle (1);
\endscope
% outline
\draw (0.35, 0) node [text=black,right] {65} % intersection
      (0,0) circle (1) (0,1)  node [text=black,above] {EP} node [text=black,below] {1} 
      (1,0) circle (1) (1,1)  node [text=black,above] {TP} node [text=black,below] {0} ;
\end{tikzpicture}

\begin{tikzpicture}[fill=gray]
% left hand
\scope
\clip (-2,-2) rectangle (2,2)
      (1,0) circle (1);
\fill (0,0) circle (1);
\endscope
% right hand
\scope
\clip (-2,-2) rectangle (2,2)
      (0,0) circle (1);
\fill (1,0) circle (1);
\endscope
% outline
\draw (0.35, 0) node [text=black,right] {61} % intersection
      (0,0) circle (1) (0,1)  node [text=black,above] {EP} node [text=black,below] {5} 
      (1,0) circle (1) (1,1)  node [text=black,above] {FST} node [text=black,below] {0} ;
\end{tikzpicture}


\begin{tikzpicture}[fill=gray]
% left hand
\scope
\clip (-2,-2) rectangle (2,2)
      (1,0) circle (1);
\fill (0,0) circle (1);
\endscope
% right hand
\scope
\clip (-2,-2) rectangle (2,2)
      (0,0) circle (1);
\fill (1,0) circle (1);
\endscope
% outline
\draw (0.35, 0) node [text=black,right] {61} % intersection
      (0,0) circle (1) (0,1)  node [text=black,above] {EP} node [text=black,below] {5} 
      (1,0) circle (1) (1,1)  node [text=black,above] {COTT} node [text=black,below] {0} ;
\end{tikzpicture}

\end{multicols}





%%% SECOND ROW

\begin{multicols}{3}


    \begin{tikzpicture}[fill=gray]
% left hand
\scope
\clip (-2,-2) rectangle (2,2)
      (1,0) circle (1);
\fill (0,0) circle (1);
\endscope
% right hand
\scope
\clip (-2,-2) rectangle (2,2)
      (0,0) circle (1);
\fill (1,0) circle (1);
\endscope
% outline
\draw (0.35, 0) node [text=black,right] {64} % intersection
      (0,0) circle (1) (0,1)  node [text=black,above] {FSE} node [text=black,below] {1} 
      (1,0) circle (1) (1,1)  node [text=black,above] {TP} node [text=black,below] {1} ;
\end{tikzpicture}




\begin{tikzpicture}[fill=gray]
% left hand
\scope
\clip (-2,-2) rectangle (2,2)
      (1,0) circle (1);
\fill (0,0) circle (1);
\endscope
% right hand
\scope
\clip (-2,-2) rectangle (2,2)
      (0,0) circle (1);
\fill (1,0) circle (1);
\endscope
% outline
\draw (0.35, 0) node [text=black,right] {61} % intersection
      (0,0) circle (1) (0,1)  node [text=black,above] {FSE} node [text=black,below] {4} 
      (1,0) circle (1) (1,1)  node [text=black,above] {FST} node [text=black,below] {0} ;
\end{tikzpicture}


\begin{tikzpicture}[fill=gray]
% left hand
\scope
\clip (-2,-2) rectangle (2,2)
      (1,0) circle (1);
\fill (0,0) circle (1);
\endscope
% right hand
\scope
\clip (-2,-2) rectangle (2,2)
      (0,0) circle (1);
\fill (1,0) circle (1);
\endscope
% outline
\draw (0.35, 0) node [text=black,right] {61} % intersection
      (0,0) circle (1) (0,1)  node [text=black,above] {FSE} node [text=black,below] {4} 
      (1,0) circle (1) (1,1)  node [text=black,above] {COTT} node [text=black,below] {0} ;
\end{tikzpicture}


\end{multicols}

\caption{GPT 4 Refactory}
\end{figure*}

\end{comment}


 \begin{table*}[t]
  \centering
  \caption{\textbf{Error Analysis for Trace-based and Error-based Prompts. AA = Assignment Addition, CMP=Comparison, AEM=Assignment Expression Modification, BCM= Branch Condition Modification, CBA=Condition Branch Addition, CBD=Condition Branch Deletion, CEE= Condition Expression Expansion, CEM=Condition Expression Modification, IM=Initialization Modification, LCM=Loop Condition Modification, MOM=Math Operator Modification ,MCA=Method Call Addition, MCM=Method Call Modification, MCPM=Method Call Parameter Modification, REM= Return Expression Modification , TM= Type Modification, VM=Variable Modification, CBM=Condition Branch Modification, DSA=Declaration Statement Addition, MCPA=Method Call Parameter Addition, MCPD= Method Call Parameter Deletion}}
%\label{tab:Per_c10_2}
  \resizebox{0.98\textwidth}{!}{
    \begin{tabular}{c|cl|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|}
    \toprule
    Model & Dataset & CMP& AA & AEM & BCM&   CBA &  CBD &  CEE &  CEM &  IM&  LCM & MOM & MCA & MCM& MCPM &REM&TM &VM& CBM&DSA&MCPA&MCPD\\
    \midrule
    \multirow{8}[1]{*}{GPT-3.5} & \multirow{4}[1]{*}{Refactory} & EP>TP &   \ApplyColorIfNeeded{0}  &   \ApplyColorIfNeeded{0}   &   \ApplyColorIfNeeded{0}    &  \ApplyColorIfNeeded{0}   &   \ApplyColorIfNeeded{0}    &   \ApplyColorIfNeeded{0}   &  \ApplyColorIfNeeded{0}     & \ApplyColorIfNeeded{0}      &  \ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{0} &\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}\\
    &  & TP>EP &        \ApplyColorIfNeeded{0}  &   \ApplyColorIfNeeded{0}   &   \ApplyColorIfNeeded{0}    &  \ApplyColorIfNeeded{0}   &   \ApplyColorIfNeeded{0}    &   \ApplyColorIfNeeded{0}   &  \ApplyColorIfNeeded{0}     & \ApplyColorIfNeeded{0}      &  \ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{0} &\ApplyColorIfNeeded{2}& \ApplyColorIfNeeded{2}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}   &\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}\\ 
    
    &  & FSE>FST & \ApplyColorIfNeeded{0}  &   \ApplyColorIfNeeded{0}   &   \ApplyColorIfNeeded{1}    &  \ApplyColorIfNeeded{0}   &   \ApplyColorIfNeeded{0}    &   \ApplyColorIfNeeded{0}   &  \ApplyColorIfNeeded{0}     & \ApplyColorIfNeeded{1}      &  \ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{1} &\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{2}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}\\
     &  & FST>FSE &       \ApplyColorIfNeeded{0}  &   \ApplyColorIfNeeded{0}   &   \ApplyColorIfNeeded{0}    &  \ApplyColorIfNeeded{0}   &   \ApplyColorIfNeeded{0}    &   \ApplyColorIfNeeded{0}   &  \ApplyColorIfNeeded{0}     & \ApplyColorIfNeeded{0}      &  \ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{0} &\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}\\
\cline{2-23}

    
     & \multirow{4}[1]{*}{HumanEvalJ} &  EP>TP &   \ApplyColorIfNeeded{0}  &   \ApplyColorIfNeeded{1}   &   \ApplyColorIfNeeded{0}    &  \ApplyColorIfNeeded{1}   &   \ApplyColorIfNeeded{0}    &   \ApplyColorIfNeeded{0}   &  \ApplyColorIfNeeded{3}     & \ApplyColorIfNeeded{0}      &  \ApplyColorIfNeeded{2}&\ApplyColorIfNeeded{1}& \ApplyColorIfNeeded{3} &\ApplyColorIfNeeded{1}& \ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{0}\\
    &  & TP>EP &        \ApplyColorIfNeeded{0}  &   \ApplyColorIfNeeded{0}   &   \ApplyColorIfNeeded{0}    &  \ApplyColorIfNeeded{1}   &   \ApplyColorIfNeeded{1}    &   \ApplyColorIfNeeded{1}   &  \ApplyColorIfNeeded{1}     & \ApplyColorIfNeeded{0}      &  \ApplyColorIfNeeded{2}&\ApplyColorIfNeeded{2}& \ApplyColorIfNeeded{2} &\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{3}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{3}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{1}\\ 
    
    &  & FSE>FST & \ApplyColorIfNeeded{0}  &   \ApplyColorIfNeeded{2}   &   \ApplyColorIfNeeded{0}    &  \ApplyColorIfNeeded{2}   &   \ApplyColorIfNeeded{0}    &   \ApplyColorIfNeeded{2}   &  \ApplyColorIfNeeded{3}     & \ApplyColorIfNeeded{0}      &  \ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{1}& \ApplyColorIfNeeded{2} &\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{4}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{2}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{0}\\
     &  & FST>FSE &       \ApplyColorIfNeeded{0}  &   \ApplyColorIfNeeded{1}   &   \ApplyColorIfNeeded{0}    &  \ApplyColorIfNeeded{1}   &   \ApplyColorIfNeeded{0}    &   \ApplyColorIfNeeded{0}   &  \ApplyColorIfNeeded{2}     & \ApplyColorIfNeeded{3}      &  \ApplyColorIfNeeded{2}&\ApplyColorIfNeeded{3}& \ApplyColorIfNeeded{2} &\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{2}&\ApplyColorIfNeeded{3}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}\\
     \midrule
     \multirow{8}[1]{*}{GPT-4} & \multirow{4}[1]{*}{Refactory} & EP>TP &   \ApplyColorIfNeeded{0}  &   \ApplyColorIfNeeded{0}   &   \ApplyColorIfNeeded{0}    &  \ApplyColorIfNeeded{0}   &   \ApplyColorIfNeeded{0}    &   \ApplyColorIfNeeded{0}   &  \ApplyColorIfNeeded{0}     & \ApplyColorIfNeeded{0}      &  \ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{0} &\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}\\
    &  & TP>EP &        \ApplyColorIfNeeded{0}  &   \ApplyColorIfNeeded{0}   &   \ApplyColorIfNeeded{0}    &  \ApplyColorIfNeeded{0}   &   \ApplyColorIfNeeded{0}    &   \ApplyColorIfNeeded{0}   &  \ApplyColorIfNeeded{0}     & \ApplyColorIfNeeded{0}      &  \ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{0} &\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}   &\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}\\ 
    
    &  & FSE>FST & \ApplyColorIfNeeded{0}  &   \ApplyColorIfNeeded{0}   &   \ApplyColorIfNeeded{1}    &  \ApplyColorIfNeeded{0}   &   \ApplyColorIfNeeded{0}    &   \ApplyColorIfNeeded{0}   &  \ApplyColorIfNeeded{0}     & \ApplyColorIfNeeded{1}      &  \ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{2} &\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}\\
     &  & FST>FSE &       \ApplyColorIfNeeded{0}  &   \ApplyColorIfNeeded{0}   &   \ApplyColorIfNeeded{0}    &  \ApplyColorIfNeeded{0}   &   \ApplyColorIfNeeded{0}    &   \ApplyColorIfNeeded{0}   &  \ApplyColorIfNeeded{0}     & \ApplyColorIfNeeded{0}      &  \ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{0} &\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}\\
\cline{2-23}

    
     & \multirow{4}[1]{*}{HumanEvalJ} & EP>TP &   \ApplyColorIfNeeded{1}  &   \ApplyColorIfNeeded{1}   &   \ApplyColorIfNeeded{0}    &  \ApplyColorIfNeeded{3}   &   \ApplyColorIfNeeded{1}    &   \ApplyColorIfNeeded{1}   &  \ApplyColorIfNeeded{1}     & \ApplyColorIfNeeded{2}      &  \ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{2} &\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}\\
    &  & TP>EP &     \ApplyColorIfNeeded{0}  &  \ApplyColorIfNeeded{1}  &   \ApplyColorIfNeeded{1}    &  \textcolor{white}{\ApplyColorIfNeeded{6}}   &  \ApplyColorIfNeeded{1}  &    \ApplyColorIfNeeded{0}   &  \ApplyColorIfNeeded{2}    & \ApplyColorIfNeeded{2}      &  \ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{1} &\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{3}&\ApplyColorIfNeeded{2}&\ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}\\
    &  & FSE>FST &     \ApplyColorIfNeeded{1}  &   \ApplyColorIfNeeded{2}    &   \ApplyColorIfNeeded{1}    &  \ApplyColorIfNeeded{1}     &   \ApplyColorIfNeeded{0}    &    \ApplyColorIfNeeded{1}   &  \ApplyColorIfNeeded{2}     & \ApplyColorIfNeeded{4}      &  \ApplyColorIfNeeded{4}&\ApplyColorIfNeeded{2}& \ApplyColorIfNeeded{0} &\ApplyColorIfNeeded{1}& \ApplyColorIfNeeded{2}&\ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{3}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}\\
     &  & FST>FSE &     \ApplyColorIfNeeded{1}  &   \ApplyColorIfNeeded{0}    &   \ApplyColorIfNeeded{0}    &  \ApplyColorIfNeeded{2}     &   \ApplyColorIfNeeded{1}    &    \ApplyColorIfNeeded{0}   &  \ApplyColorIfNeeded{1}     & \ApplyColorIfNeeded{2}      &  \ApplyColorIfNeeded{2}&\ApplyColorIfNeeded{1}& \ApplyColorIfNeeded{2} &\ApplyColorIfNeeded{0}& \ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{1}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}&\ApplyColorIfNeeded{0}\\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:RQ3}%
\end{table*}%

In this research question, we discuss if any type of bug can be solved exclusively when using execution traces. In the previous sections, we find that adding execution traces does not provide any guarantee for improving the program repair capability in the models. However, it is important to understand if any specific bugs are only solved using trace-based prompts. For that purpose, we compare programs fixed by different error-based and trace-based prompts and produce Venn diagram that can show the number of faulty programs fixed by only that prompt type. However, our main objective is to analyze the Venn diagrams between EP-TP and FSE-FST across different datasets and GPT. 

Figure \ref{fig:rq3_java_gpt3.5}, \ref{fig:rq3_py_gpt3.5}, \ref{fig:rq3_java_gpt4} and \ref{fig:rq3_py_gpt4} show our findings (Last three figures are in appendix). For HumanEval-Java dataset, it is evident that trace-based programs fix a significant number of faulty programs that are not solved by error-based prompts. Specifically, TP always solves more number of unique programs than EP.


%for GPT-4 model, the numbers are higher. For example, for GPT-4 model, FSE and TP prompts both help to fix 112 programs; however, 17 of the faulty programs are only solved by FSE or TP prompts. 

On the contrary, for Refactory dataset, few programs are only solved by trace-based prompts. These results further support the claim that GPT models can not utilize the execution traces to fix programs in the Refractory dataset.  

 
\begin{center}
\begin{tcolorbox}[colback=gray!10,%gray background
                  colframe=black,% black frame colour
                  width=7.5cm,% Use 8cm total width,
                  arc=1mm, auto outer arc,
                  boxrule=0.9pt,
                 ]
 \textbf{RQ2 Summary.} For HumanEval-Java dataset, a significant number of programs are fixed only by trace-based prompts.
\end{tcolorbox}
\end{center}

\subsection{RQ3. Which types of bugs require specific program execution traces in order to be fixed?}


%\def\cca#1{\cellcolor{black!#10}\ifnum #1>5\color{white}\fi{#1}}
In this section, we discuss different types of bugs present in the unique faulty programs repaired by error-based (EP, FSE) and trace-based prompts (TP, FST). Table \ref{tab:RQ3} shows our results. The error types mentioned in the table are operations that must be performed on the faulty program to get the correct program based on the taxonomy introduced in HumanEval-Java. For each row, the term $X>Y$ focuses on the error types in the programs repaired by the specific type of prompt $X$, but not repaired by the prompt type $Y$.

For the HumanEval-Java dataset on GPT-4, we could find that more errors belonging to error types like Conditional Branch Addition and Method Call Parameter Modification have been solved uniquely by TP against EP. Additionally, Method Call Addition error types have been solved uniquely by FST against FSE. However, for the HumanEval-Java dataset on GPT-3.5, we do not find a similar pattern. TP could repair more number of errors belong to error types like Return Expression Modification and Variable Modification (against EP). On the other hand, FST could solve more errors belonging to Initialization Modification, Loop Condition Modification, and Type Modification.

Unlike HumanEval-Java, Refactory does not include annotations of bug types present in a given faulty program. Thus, we had to manually classify bug types by analyzing the diffs to the closest working program by edit distance. Consequently, for only half of the considered Refactory programs bug types could be clearly identified. The reason is most of the faulty programs from this dataset have logical flaws not localized to particular statements and need extensive modification to obtain the correct solution. Among the analyzed programs, we find error types related to method calls are solved more frequently by TP with GPT-3.5.
%, and Method Call Addition have been solved uniquely by TP and FST against EP and FSE, respectively.

%have been used to induce fault in HumanEval-Java dataset.  

\begin{center}
\begin{tcolorbox}[colback=gray!10,%gray background
                  colframe=black,% black frame colour
                  width=7.5cm,% Use 8cm total width,
                  arc=1mm, auto outer arc,
                  boxrule=0.9pt,
                 ]
 \textbf{RQ3 Summary.} We find that some of
the prompt types can be more effective at handling
a specific type of error than other error types. However, this observation is also model-dependent.
\end{tcolorbox}
\end{center}

==> sections/introduction.tex <==
%\section{Introduction}

% The inception of Large Language Models (LLMs) has revolutionized applications that span across different data modalities, like vision, speech, and text --- including natural language as well as source code. 
% Although fundamentally language models learn to estimate the probabilities of words sequences, training them on massive text corpora using a self-supervised objective, has been shown to endow them with rich language capabilities across a range of tasks. 
% %LLMs can be divided based on the type of corpora used to train them into General Language Models (GLM) --- capable of handling natural language-based tasks, in one or multiple languages; and  Code Language Models (CLM) --- designed specifically for programming-related tasks. 
% Although code-specific LLMs (CLMs) have been proposed, since the release of powerful generic purpose LLMs, such as GPT ~\cite{ouyang2022training, OpenAI2023GPT4TR}, it has been observed that these models can even outperform CLMs on certain coding tasks. 

Automatic program repair (APR) is one of the most challenging code automation tasks.
While trivial bugs can be easily detected by examining the source code, many real-world software defects and vulnerabilities are quite subtle and require a deep understanding of the execution and interactions between different elements of the program.
Traditionally, software engineers and security experts have relied on specialized tools, such as debuggers and profilers, to interactively step through a program's execution, examine variable states, and monitor hardware usage to identify and fix defects.
% APR techniques have improved software reliability by transforming defective programs into correctly functioning ones. Deep Learning (DL) approaches have been popular to repair defective programs. DL approaches learn from training data, which is usually comprised of both defective and correctly functional programs. DL-based techniques~\cite{li2020dlfix,drain2021deepdebug} have successfully outperformed traditional APR techniques. However, recent work shows that there is a gap for DL-based APR research to be used in practice~\cite{noller2022trust}. Recently, other approaches like LLMs have been considered for APR.
% 
\begin{figure}[t]
\begin{minted}[fontsize=\small,linenos,firstnumber=9,tabsize=2,numbersep=3mm, xleftmargin=5mm,breaklines]{Python}
### Buggy Program:
def search(x, seq):
    index = 0
    def helper(index):
        if not seq:
            return 0
        elif x <= seq[index]:
            return index
        else:
            if index + 1 >= len(seq):
                return index + 1
            else:
                return helper(index+1)

### Failing test case:
result = search(42, (-5, 1, 3, 5, 7, 10))
assert result == 6,                    'Expected 6 but got %s' % result
AssertionError: Expected 6 but got None

### Execution trace:
Starting var:.. x = 42
Starting var:.. seq = (-5, 1, 3, 5, 7, 10)
call        10 def search(x, seq):
line        11     index = 0
New var:....... index = 0
line        12     def helper(index):
New var:....... helper = <function search.<locals> .helper at 0x7fd455b89040>
return      12     def helper(index):
Return value:.. None
\end{minted}
\label{fig:trace-example}
\caption{Example buggy program, a failing test case and its execution trace. While the failure message simply indicates the output is wrong, the execution trace provides a detailed explanation how it was produced.}
\end{figure}
% 
% Despite the impressive performance of LLMs at generative code tasks, in performing APR they are limited to static analysis of the provided program and have little insight into its execution, which could hinder their bug-fixing ability \cite{ding2023traced}.
With the advent of LLMs showing impressive performance at generative code tasks, 
it remains an open question whether the static view of the code alone is sufficient for solving APR effectively.
On the one hand, LLMs have been shown to match or even outperform specialized deep learning-based and traditional APR tools ~\cite{xia2022less,jiang2023impact}. 
On the other hand, there is work suggesting potential blind spots in using LLMs for APR ~\cite{tian2023chatgpt} and highlighting limitations in reasoning about code ~\cite{invariants52366}.
%whether they are able to reason about program execution from the code alone \cite{sutton}
% However, researchers have not found significant evidence that LLMs like GPT can reason properly. For example \cite{valmeekam2023large} show that even on the simple blocks world task GPT is not capable of generating meaningful plans based on the natural language descriptions of the domain and the starting and goal states. 
% On the other hand, the ability to step through or trace a program's execution, provided by most IDEs, has been an indispensable tool for human programmers to find and fix bugs. 

Thus, in this work, we aim to remedy this potential blind spot by augmenting standard APR prompts with program execution traces. 
% In this work, our objective is to evaluate GPT model's capability to repair a faulty program using program execution traces.
% However, execution traces have not been considered for repairing program using LMs.
%
% Although program execution traces have not been significantly considered for improving APR using LLMs, 
% Recent work looked into augmenting static code with execution information for APR using LLMs. SelfAPR \cite{ye2022selfapr} proposes to use compiler and test diagnostics during self-supervised training of the language model for APR.  
% Self-Debug \cite{chen2023teaching} proposes to generate execution traces directly from the LLM as part of solving the APR task. 
% Additionally, several works have proposed the use of execution traces for pretraining code LLMs. In \cite{ding2023traced, liu2023code}, authors train a language model to predict the execution traces and later evaluate the models on different downstream tasks. 
% Finally, Bouzenia et al. ~\cite{bouzenia2023tracefixer} incorporate execution traces into LLM finetuning and show improvement on APR tasks over the code-only baseline.
% To the best of our knowledge, all of these works do not consider the effect of putting execution traces in the prompt of a pretrained LLM. In this work, our objective is to evaluate GPT model's capability to solve a generative task (APR) without finetuning, by providing the execution trace as part of the prompt during inference. 
%
%
%
%
%several works have proposed the use of execution traces for pretraining CLMs. In \cite{ding2023traced, liu2023code}, authors train a language model to predict the execution traces and later evaluate the models on different downstream tasks. To our knowledge, none of the works propose leveraging program execution traces at inference time. 
% Also, neither of the works considers any generative task to solve. 
%In this work, our objective is to evaluate GPT model's capability to solve a generative task (APR) without finetuning, by providing the execution trace as part of the prompt during inference. For the purpose of evaluating our approach, we select two recent APR datasets: Refactory~\cite{hu2019re} and HumanEval-Java~\cite{jiang2023impact}. 
%
%To use the 
% To evaluate GPT model's capability reason about program execution, w
%We frame our work in terms of three research questions (RQs). The first RQ focuses on determining if the GPT model's capability is improved after adding execution traces in the prompt. Specifically, we compare the GPT model's program repairing capability given prompt with traces against the prompts with assertion error messages and program-only prompts.  Additionally, we focus on feeding enriched prompts (chain-of-thought and extended) to GPT models to investigate the impact of enriched prompts on trace-based prompts. While we find that traces could not improve GPT-3.5 model's capability in repairing programs, GPT-4 has shown promising results in repairing programs using traces for HumanEval-Java dataset.
We frame our work in terms of three research questions (RQs). 

In RQ1 (Section \ref{sec:RQ1}), our objective is to quantify the gains from incorporating execution traces into the APR prompt over the prompts only containing the failing test case as well as the 
trace-free chain-of-thought prompting baseline~\cite{chen2023teaching}.
% compare the impact of execution traces generated by GPT with the impact of execution traces generated during runtime. 
% Chen et al~\cite{chen2023teaching} have shown that generating execution traces from LLMs can lead to better repairing of programs. 
% Our objective is to analyze if replacing the LLM-generated execution traces with runtime execution traces would improve the program repairing capability of GPT or not. We also compare the aforementioned trace-based prompting techniques with only error message-based prompting techniques. 
We find that simply adding the execution trace does not consistently outperform trace-free prompts.

%In the second RQ, we focus on feeding enriched prompts (chain-of-thought, few-shot and extended) to GPT models to investigate the impact of enriched prompts on trace-based and error-based prompts. The chain-of-thought prompt's objective is to search for the error location first and then find the repaired program. We find that while using few-shot prompts could significantly improve the program repairing capability for HumanEval-Java dataset, chain-of-thought based prompts produce worse performance in GPT model's w.r.t repairing program.

%In the second RQ, the focus is to find out if specific programs can only be repaied by using trace-based prompts or not. For this purpose, we use Venn diagrams to show which of the fixed programs are solved only by trace-based prompts. We find that for HumanEval-Java dataset, a significant number of fixed programs are only solved by trace-based prompts. 

To inform a more finegrained approach, in RQ2 (Section \ref{sec:RQ2}), we analyze the relationship between trace complexity and the likelihood of the LLM producing a working fix.
% the focus is on analyzing how the complexity of the runtime execution traces can impact the GPT models' program-repairing capability. 
To measure this complexity, we consider two parameters: trace length and the number of variable modifications. 
We find that the effectiveness of trace-based prompts decreases with the growing length and number of variable assignments.% if the trace complexity is lower, putting a trace in a prompt is more likely to repair faulty programs. 

%In the third RQ, we analyze the bugs uniquely solved by trace-based prompts based on the type of error introduced. For this purpose, we consider 20 types of errors introduced in HumanEval-Java dataset~\cite{jiang2023impact}. We find that some of the prompt types can be more effective at handling a specific type of error than other error types.
%\textcolor{red}{TODO}

Motivated by this finding, in RQ3 (Section \ref{sec:RQ3}), we aim at improving the consistency of trace-based APR by experimenting with three different representations of execution traces: traces in a collated format, LLM-optimized traces, and a trace representation conditionally selected based on querying the LLM's confidence. 
We find that LLM-optimized trace-based prompts provide the most consistent results with respect to program repair. 

We additionally perform two follow-up studies: in the first, we compare our trace-based prompting approach with a fine-tuned baseline inspired by TraceFixer \cite{bouzenia2023tracefixer}; and in the second one, we directly probe the LLM on two trace understanding tasks.
%Finally in the fourth RQ, we discuss if fine-tuning a small-sized model is better for program repair than prompting GPT models. Our finding shows that prompting GPT models with traces outperforms fine-tuned models for program repairing.
% Our work makes the following contributions: 

% \begin{itemize}

%     \item\textbf {Problem Characterization.} Our work is the first work to characterize the effect of program execution traces on GPT model's capability. 
%     \item\textbf {Experimentation.} We investigate GPT model's capability to reason about program execution extensively through three research questions.
%      \item\textbf {Findings.} For research questions, we discuss the findings thoroughly, which can help software developers/researchers to investigate furthermore about LLM's program repairing capability. 

% \end{itemize}
% For the purpose of evaluating our approach, we select three recent APR datasets: Refactory~\cite{hu2019re}, RunBugRun~\cite{prenner2023runbugrun} and HumanEval-Java~\cite{jiang2023impact}. 

%\textbf{A very short paragraph: the flow of the paper "The rest of the paper is organized as follows: In Section 2, we introduce the ........."}
The rest of the paper is organized as follows. In Section \ref{sec:back}, we discuss the related work and how it differs from our approach.
% about LLM's reasoning capability and APR using LLMs. 
Section \ref{sec:rq12} details our methodological setup and covers RQ1 and RQ2. 
Section \ref{sec:rq3} covers RQ2 and in Section \ref{sec:disc}, we discuss the additional studies.



%Our finding suggests that prompts with traces perform better than prompts with errors w.r.t repairing programs.

%Traditionally, LMs can be divided into Code Language Models (CLMs) and Generic Language Models (GLM). CLMs are specifically designed for programming language related tasks, while GLMs are also capable handling natural language based tasks. Recently, multiple works have evaluated the APR capability of LMs~\cite{}.


%\section{Motivating Example}
%\noindent
%\begin{figure*}

%\end{figure*}



==> sections/limitation.tex <==
Our work has the following limitations.

\noindent\textbf{Generating Execution Trace.} As mentioned in Section \ref{sec:rq12}, we find that not all Python programs can generate execution traces, especially if a file contains multiple programs. Similarly, for Java, to generate an execution trace, we needed to transform the program. In that process, we could not transform seven programs out of 164 programs. 

\noindent\textbf{Focusing on the GPT Family of Models.} In this work, we have focused on only GPT-3.5 and GPT-4 models, while there are other LLMs (\textit{e.g.,} Llama2), which can be investigated for reasoning about execution traces.

\noindent\textbf{Using Single Sample per Prompt.} In this work, we queried the GPT API only once per prompt, whereas it is common in the literature to obtain multiple samples and report either the maximum or average pass rate. However, due to the test-case specific nature of our prompts, we still obtain multiple fixes for the same bug albeit given multiple prompt variations. Out of practical considerations, we opted not to introduce an additional level of complexity. Nonetheless, results could be more stable if we had multiple samples per prompt.



\noindent\textbf{Analyzed Languages.} In this work, only consider Java and Python as languages. However, these two languages are very popular in software development.

\noindent\textbf{Limitations of Datasets Studied}. We aimed at choosing sufficiently diverse datasets, both in terms of language, as well as the nature of the underlying code and bugs. Yet, some of those differences could be confounding to our conclusions, for example, the fact that bugs were manually introduced in HumanEval-Java. A more extensive investigation across a large set of dataset would help strengthen the claims made in this paper.


==> sections/methodology.tex <==
%\todo{describe how we use execution traces to improve APR}

\label{sec:method}
In formulating APR prompts, we follow the instruction template for complete function generation used by Xia et al. (\citeyear{ICSE10172803}), expanding it to incorporate additional pertinent information for fixing a bug. First, in addition to including the buggy function itself we find it helpful to include a failing test case, to give the LLM a hint about the function's desired vs actual output.
In our preliminary experiment such prompts performed always better than program-only prompts\footnote{Furthermore, we explored the option of including all failing test cases in the same prompt, however that did not provide a lift compared to a single test case, and overall performed slightly worse. We hypothesize multiple test cases could be more helpful for program generation to help define the space of valid solutions, whereas in APR the buggy function itself provides a bulk of information for fixing a bug, and a single failing test case, while inexhaustive, is generally sufficient for setting the LLM on the right path to finding a fix.}. Our general conviction is that detailed step-by-step traces of program's execution will provide the LLM with even better visibility into how the result emerges, significantly increasing the chances of a correct fix. We explore several different trace formats discussed in the next sections.

\subsection{Deterministic Execution Traces} 
As the program is being executed, it is possible to step through it programmatically, while also capturing every change to the function's variables, akin to interactive debugging. PySnooper\cite{pysnooper} library for Python provides this functionality via a decorator that can be added to a function of interest to automatically log state changes, such as variable initialization and modification, subroutine calls, returned values, and runtime exceptions. Crucially, each state change reference a specific line of code on which it occurred. Examples of execution traces are given in the Appendix \ref{subsec:TP}. Before appending traces to the prompt we perform basic postprocessing, including the removal of timestamps and stripping of terminal formatting command sequences.




 % The deterministic execution traces are traces generated through program execution using library. The objective of generating deterministic execution traces is to help GPT models understand the program flow. To fulfill that objective, we focus on generating execution traces that include the modification in different variable values. Different debuggers based on IDEs (\textit{e.g.,} IntelliJ\cite{intellij}) also provide different variable values on specific breakpoints (lines) to help users debug any issue. However, the selection of the breakpoint location is dependent on the end user, who might not be an expert in the programming language to correctly identify them. For that purpose, we propose to update the execution traces whenever a variable value in the program is modified.

\begin{comment}
\begin{figure}
%\begin{tabular}{@{}c@{}}
%\hspace{-2.8cm}
\begin{minipage}[h]{\linewidth}
\begin{minted}[fontsize=\small,linenos,tabsize=2,numbersep=3mm, xleftmargin=5mm,breaklines]{Python}
def search(x, seq):
    idx = 0
    def hlpr(idx):
        if not seq:
            return 0
        elif x <= seq[idx]:
            return idx
        else:
            if idx + 1 >= len(seq):
                return idx + 1
            else:
                return hlpr(idx+1)
'''Starting var:.. x = 42
Starting var:.. seq = (-5, 1, 3, 5, 7, 10)
call        1 def search(x, seq):
line        2     index = 0
New var:....... index = 0
line        3     def hlpr(index):
New var:....... helper = <function search.<locals>.helper at 0x000001ABA832FB80>
return      3     def hlpr(index):
Return value:.. None
'''
\end{minted}
\end{minipage}
\caption{Code Snippet and Corresponding Execution Trace}
\label{fig:ex}
%\end{tabular}
\end{figure}
\end{comment}
% Section \ref{subsec:TP} (In Appendix) shows a python function with the generated execution traces. The function accepts a list of tuples, where each tuple has gender and age of different persons.
% The objective of the program is to return the sorted list based on age.
% From the trace, we can find that the return value of the program is 'None' because the sort function modifies the list in place but does not return any value. 


% \subsubsection{Generating Execution Traces in Python} To generate execution traces in Python, we have used PySnooper\cite{pysnooper} library. PySnooper prints all the variable changes in the program, given the correct annotation is provided. For example, to get execution trace within a function '@PySnooper.snoop()' annotation has to be added before the function declaration. However, PySnooper-generated traces have timestamps of executed instructions in the trace, which can add confusion to the prompt. Hence, before adding traces to the prompt, we remove the additional timestamps from the traces.

% However, automating the process to get execution trace using PySnooper can lead to losing some of the traces. For automation, we add the annotation before the first function of the file. However, for datasets like Refactory~\cite{hu2019re}, where solutions can consist of multiple functions within one file, which can lead to the loss of traces for certain functions. Because of this reason, we used approximately 100 programs (instead of 164) in Refactory during evaluation.


% \subsubsection{Generating Execution Traces in Java} 
For generating execution traces in Java, we did not come across any library similar to PySnooper and thus had to implement our own utility leveraging Java's aspect-oriented framework AspectJ ~\cite{spring}.
While logging of state changes is one of the integral capabilities of AspectJ, its scope is limited by default to only class level variables, which would skip non-class member local variables from the resulting execution trace.

% \begin{figure}
%   \begin{center}
%     \includegraphics[width=0.48\textwidth]{figures/Codeplan.drawio-3.pdf}
%   \end{center}
%   \caption{Overview of Trace Generation For Java Program}
%   \label{fig:java}
% \end{figure}

\begin{figure}
  \begin{center}
    \includegraphics[width=0.5\textwidth]{figures/CondT.drawio.pdf}
  \end{center}
  \caption{The Flow of Conditional Selection of Traces}
  \label{fig:cond}
\end{figure}

To overcome limitation, we automatically refactor each buggy program in the dataset by declaring each of its local variable as a class member and initializing them with the corresponding the local variable's value. This transformation allows AspectJ to log all variables from the original program we are interested in.  Examples of Java traces are given in the Appendix.
%Figure \ref{fig:java} shows the overview of creating Java traces. 





==> sections/motivated.tex <==
\section{Motivating Example}
\label{sec:motivated}
We show the motivation for analyzing the effect of program execution traces on GPT models through an example. HumanEval-Java dataset has the following program GET\_ODD\_COLLATZ where the task is explained as: \textit{Given a positive integer n, return a sorted list that has the odd numbers in collatz sequence.
The Collatz conjecture is a conjecture in mathematics that concerns a sequence defined
    as follows: start with any positive integer n. Then each term is obtained from the 
    previous term as follows: if the previous term is even, the next term is one half of 
    the previous term. If the previous term is odd, the next term is 3 times the previous
    term plus 1. The conjecture is that no matter what value of n, the sequence will always reach 1.
Note: 
        1. Collatz(1) is [1].
        2. returned list sorted in increasing order.}




Figure \ref{fig:motiv} shows an example, where a faulty version of the program is written (Line 11, 13 and 14). We create two prompts based on the faulty program and send the prompt to GPT3.5 \cite{ouyang2022training}. The first prompt consists of the faulty program, a failing test case and the function's execution trace (Figure \ref{fig:motiv}), while the second prompt does not have the execution trace in it. We found that GPT 3.5 successfully fixes the bug when provided with the full prompt, but fails when the prompt omits the execution trace. Hence, the example provides a preliminary indication that LLMs could use execution traces to fix faulty programs more effectively.


%We generated synthetic Python functions consisting of simple arithmetic operations accompanied by an assert statement about the function's returned value, while replacing the actual returned value in the function's body with a mask.Based on the value in the assert statement, only one of the function's variables is the correct answer for the mask.Yet, PL-Bart's top-5 predictions for the mask were virtually unaffected by the different values plugged into the assert statement. It predicts the most common tokens and is only correct about 30\% of the time (3-way classification), even after finetuning.Additionally, we generated adversarial examples where the most recent token before the return statement is never the answer and observed PL-Bart's performance drop further.

%We show that this task can be solved perfectly by an algorithm that keeps track of variable's values at every step of the program.To demonstrate this task can feasibly be solved by a model with some capability for reasoning about data dependencies among variables, we train a supervised model based on Memory Networks.We used gold values for the mask, as well as k ``supporting facts'' -- indices of lines that the resulting value depends on, as labels.Even with k=3, which does not capture full data dependencies, this model outperforms PL-Bart by more than two-fold.In addition, we outperform a GPT model on the same task in zero-shot as well as few-shot settings (albeit by a narrower margin).

\begin{figure}
\begin{minipage}{\columnwidth}
    %\begin{mybox}{Prompt}
    
    \begin{minted}[fontsize=\small,linenos,tabsize=2,numbersep=3mm, xleftmargin=5mm,breaklines]
{Java}
//### Provide a fix for the buggy function.
//### Buggy Function:
package org.humaneval;
import java.util.ArrayList;
import java.util.Collections;
public class GET_ODD_COLLATZ {
  public ArrayList<Integer> get_odd_collatz(  int temp_n){
    this.n=temp_n;
    ArrayList<Integer> temp_result=new ArrayList<>();
    this.result=temp_result;
    if ((n % 2) == 1)     result.add(n);
    while (n >= 1) {
      if ((n % 2) == 1)       n/=2;
 else       n=3 * n + 1;
      if ((n % 2) == 1)       result.add(n);
    }
    Collections.sort(result);
    return result;
  }
  int n;
  ArrayList<Integer> result;
}
//### Failing Test Case:
//test_0(org.test.TEST_GET_ODD_COLLATZ): expected:<[1, 5, 7, 11, 13, 17]> but was:<[1, 3, 7, 15, 21, 31, 43]>
//### Function Execution Trace:..............................

    \end{minted}
\end{minipage}
\caption{Prompt for Motivating Example}
\label{fig:motiv}
%\end{tabular}
\end{figure}

==> sections/related-work.tex <==
\subsection{Automatic Program Repair with LLMs}
Code LLMs hold great promise for APR as they can be generically pre-trained on a code corpus, without requiring labeled bugs datasets or language-specific tuning; however, the big question is how well they measure up with specialized APR systems.
% SOTA APR with LLM and DL
Several recent papers examined performance of code LLMs at the APR task against state of the art specialized deep learning-based and traditional template based tools. 

% 2.	This year’s survey of LLM for APR performance https://lingming.cs.illinois.edu/publications/icse2023a.pdf, covering Codex, GPT-J/Neo/X, InCoder, CodeT5 on Defects4J, QuixBugx, ManyBugs
In \cite{ICSE10172803}, the authors evaluate 9 code LLMs of various sizes across 5 benchmarks in 3 APR settings: patch generation from scratch, infilling given prefix and suffix, and predict single line fix.
% outperform APR tools even without finetuning (DL and traditional) REALLY?
% all LLMs worse than DL on Defects except Codex
% scaling model size improves repair quality but codex > neo x
They find, through prompting alone and without task-specific finetuning, larger code LLMs such as Codex \cite{} and GPT-NeoX \cite{} are able to perform on par or outperform state of the art deep learning models, such as AlphaRepair \cite{} and traditional tools such as TBar \cite{}. 
In addition to the LLM size, they observe the type of prompt to be a crucial factor in the model's performance. 
% infilling and single line fixes are more accurate than complete patch generation (given gold?) -> but how localize
% in complete generation needs to determine root cause of the bug and localize it in code
% providing suffix is crucial
Specifically, infilling and single line fixes tend to be produce more accurate fixes than complete patch generation given that in the latter case the model not only needs to generate the correct fix but also autonomously localize the failure in code.
% they evaluate generative but without FIM
% in single line generation, higher syntactic error
They also underscore the importance of providing the suffix of program to the syntactic correctness of the generated fix.
Additionally, they find LLMs useful in predicting correctness and ranking of generated patches by using the entropy measure.
% LLMs can be used to rank patches or correctness checking
Finally, they show APR performance can be improved further by increasing the number of samples per program from 200 to 2000 and by including patch templates in the training. % -- something they started the paper by criticizing
% template-based APR provides good fixes but has poor generalization

% 3.	Great study by your team https://arxiv.org/pdf/2302.05020.pdf also benchmarking LLMs against DL-based systems, including Cure and Knod! 
Similarly, \cite{jiang2023impact} find code LLMs have surprisingly good APR performance out of the box compared to purpose built DL models.
% use only java datasets
On 4 Java bugs datasets they show PLBart \cite{}, CodeGen 2B \cite{}, and InCoder \cite{} fix as much as 72\% more bugs in total than popular DL-based techniques, including Recoder \cite{} and RewardRepair \cite{}, without task-specific finetuning.
% buggy line does not benefit llm
Somewhat surprisingly, they also find that providing the buggy line hurts the LLM program repairing performance, which can be explained by the misalignment with the pretraining data distribution.
% smaller models benefit from small finetuning the most up to a point then decrease
On the other hand, a moderate amount of finetuning provides further gains of over 31\% across models, whereas including beyond 50k training instances causes APR performance to degrade, which in the authors' view introduces over-reliance on buggy lines.
% they find some data leakage
It should be noted, however, that the gap in performance between LLMs and DL models is not universal across datasets: LLMs tend to fix more bugs in simpler datasets such as QuixBugs \cite{} and HumanEval-Java \cite{jiang2023impact} -- which the authors themselves introduced to address possible data leakage -- compared the more difficult Defects4J datasets, on which DL models still hold their ground compared to most non-finetuned LLMs.
% report pass@10
Still, the reported LLM performance is achieved with just 10 samples per patch, compared thousands commonly generated by DL models.

% 4.	More evaluations of Codex modifications with detailed error analysis https://arxiv.org/pdf/2205.10583.pdf
In a different study, Fan et al. \cite{fan2023automated} did a systematic analysis of bugs contained in programs generated by Codex and concluded that it lacks deep algorithm understanding despite generating plausible code, and is prone to reproducing human errors seen in the training data.
They identify error symptoms such as names referencing wrong algorithms, repeated code blocks and irrelevant helper functions.
They additionally apply APR tools such as Recoder and TBar, as well as Codex with edit mode to fix Codex generated code for LeetCode easy and medium problems.
They find that only a 20\% to 30\% of single-hunk Codex errors can be fixed with APR tools, possibly due to the majority of errors being identified as algorithm-related, as opposed to syntactic ones and simple operator and variable replacements.
% COdex e slightly outperforms when given buggy line
Codex with edit mode slightly outperforms APR tools on single hunk errors, especially when provided with fault localization, and is shown to at least in principle be able to fix multi-hunk bugs, unlike TBar and Recoder.
Finally, authors suggest combining Codex with TBar to increase the space of usable patches. 

% 5.	This paper investigates the performance of chatgpt on program repair approach (section 4.2) https://arxiv.org/pdf/2304.11938.pdf
% evaluate ChatGPT for generation and APR and summarization
Tian et al. \cite{tian2023chatgpt} investigate the performance of ChatGPT and Codex on on a range of tasks including APR, on a Python dataset called Refactory \cite{} in comparison to a semantics-based APR tool of the same name \cite{}.
ChatGPT is competitive with Refactory with 84\% top-5 success rate vs 90.8\% of Refactory 90.8 on average but, outperforms on certain problems, whereas the authors note the top-1 accuracy is only 60\%.
Despite being specialized for code, Codex lags behind with 66\% top-5.
The authors investigated the impact of including the problem description on APR performance and found while it benefitted Codex predictions for most problems, only improved ChatGPT in one scenario, while degrading in all all others. The authors attribute this to the distraction of GPT by the description which may not always be relevant to the bug on hand.
On the other hand, having more formal specification of the input and/or failing test case proved essential.


Overall, the findings in these works vary from LLMs decisively outperforming, to being on par, to even lagging behind specialized APR tools.
Multiple methodological differences could account for such discrepancy: 1) different datasets of different sizes, programs of different complexity and languages 2) different sets of models evaluated, including proprietary ones, 3) different number of samples evaluated/top-k reported )

Leakage of the test examples into the training data is the universal concern of the above works, prompting some authors to create their own datasets for unbiased evaluation.

\subsection{Reasoning about Program Execution}
% Reasoning as a transition to traces
Reasoning ability of large language models has been called into question ever since their introduction. 
For example \cite{valmeekam2023large} show that even on the simple blocks world task GPT is not capable of generating meaningful plans based on the natural language descriptions of the domain and the starting and goal states.
On the other hand, Wang et al. \cite{wang2023grammar} demonstrate a remarkable ability of LLMs to generate formulae that conform to a formal grammar formalism provided to the model.

When it comes to automatic program repair, a big question is whether to be successful at the task the model actually needs to reason about the changing state of the program's execution or it is sufficient to rely on syntactic cues learned from a sufficiently large code corpus.
In a recent work, Sutton et al. \cite{invariants52366} investigate the capacity of code LLMs for predicting program invariants.
Invariants are universal properties that are satisfied at different points of the program regardless of specific inputs, and can be thought of as an abstraction of the program state.
Their prediction from source code is challenging as traditional tools usually derive them from large collections of execution traces.
The authors pre-trained smaller versions of PaLM \cite{} on GitHub code and finetuned them on gold invariants derived from a dynamic analysis tool Daikon \cite{} applied to code competitions data.
As a result of finetuning, the models achieved scores in mid-eighties range for predicting invariants at predefined points in the program code.
Moreover, the authors noted a several point improvement when using a scratchpad strategy as opposed to single-point prediciton.
Upon qualitative examination it is found that LLMs are actually able to uncover many valid invariants that the deterministic tool missed.
Furthermore, larger LLMs tend to not only perform better but also reveal non-trivial invariants requiring multi-step reasoning. 
Additionally, they performed a preliminary zero-shot experiment with GPT-4 \cite{}, which achieved less than 50\%, leading the authors to conclude finetuning to be a crucial ingredient for learning this task.
Unfortunately, they conducted neither few-shot nor chain-of-thought prompting \cite{}, which could provide better insights into LLM's innate ability for predicting and reasoning about important program properties such as invariants.

When it comes to APR, a tool called TraceFixer \cite{bouzenia2023tracefixer} based on CodeT5 is finetuned to leverage execution traces for program repairing. The authors evaluate on one real bugs dataset and two code competition datasets, where they introduce bugs using a learned mutation model from the first dataset. They demonstrated more than 13\% improvement over the code-only baseline consistent across different top-k values on the synthetic bugs datasets, however on real bugs achieve significantly lower scores, which could indicate the model's limited generalization.

Ding et el. \cite{ding2023traced} also pretrain language models on a combination of source code with executable inputs and resulting execution traces to predict program states and execution coverage. However, their downstream task evaluations include clone detection and vulnerability detection but not program repair. Nonetheless they demonstrate steady improvement over UnixCoder. Similarly, Liu et al. \cite{liu2023code} evaluate their model pre-trained for program state prediction on the tasks of code search and code generation -- both showing strong gains when applied on top of baseline models.

% QUESTION which bugs require traces to solve?


% Reasoning about execution?

% 1.	This recent paper https://openreview.net/pdf?id=mXv2aVqUGG looks at execution traces but with a purpose of predicting program invariants rather than APR.



\subsection{Bugs Datasets}
